Assessing Visually-Continuous Corruption Robustness of Neural Networks Relative to Human Performance

While Neural Networks (NNs) have surpassed human accuracy in image classification on ImageNet, they often lack robustness against image corruption, i.e., corruption robustness. Yet such robustness is seemingly effortless for human perception. In this paper, we propose visually-continuous corruption robustness (VCR) -- an extension of corruption robustness to allow assessing it over the wide and continuous range of changes that correspond to the human perceptive quality (i.e., from the original image to the full distortion of all perceived visual information), along with two novel human-aware metrics for NN evaluation. To compare VCR of NNs with human perception, we conducted extensive experiments on 14 commonly used image corruptions with 7,718 human participants and state-of-the-art robust NN models with different training objectives (e.g., standard, adversarial, corruption robustness), different architectures (e.g., convolution NNs, vision transformers), and different amounts of training data augmentation. Our study showed that: 1) assessing robustness against continuous corruption can reveal insufficient robustness undetected by existing benchmarks; as a result, 2) the gap between NN and human robustness is larger than previously known; and finally, 3) some image corruptions have a similar impact on human perception, offering opportunities for more cost-effective robustness assessments. Our validation set with 14 image corruptions, human robustness data, and the evaluation code is provided as a toolbox and a benchmark.

==> sections/background.tex <==
\section{Background}
In this section, we present the necessary background on the metric $\Delta_v$ we use to determine visual change in images and how human recognition performance is measured through experiments. 

\subsection{Measuring Visual Change in Images}
\red{could be reduced and merge with benchmark generation + two definitions (see supp for more details)}
The metric $(\Delta_v)$, as shown in Def.~\ref{def:visual_degrade}, is proposed by Hu et. al~\cite{hu-et-al-22} to quantitatively measure the amount of visual changes in the images to human observers that is independent of particular images and transformations. Using $(\Delta_v)$ while studying human robustness removes the complexity of different transformation parameter numbers and domains; and also how transformations can impact individual images differently.

$\Delta_v$ is defined with two Image Quality Assessment (IQA) metrics, which given the original image, automatically predict the perceived image quality by measuring the perceptual ‘distance’ between the original and transformed images~\cite{hu-et-al-22}. Specifically, $\Delta_v$ uses two IQA metrics VSNR~\cite{VSNR} and VIF~\cite{VIF} for considering imperceptible and visible changes respectively~\cite{hu-et-al-22}. 

\begin{definition}
Let an image $x$, an applicable transformation $T_X$ with a parameter domain $C$ and a parameter $c\in C$, s.t. $x' = T_X(x,c)$ be given.
Visual change $\Delta_v(x,x')$ is a function defined as follows:
    {\small  \[ \begin{cases} 
      0  & $If VSNR$(x, x')= \infty \\
      &$ or VIF$(x,x')>1\\
       1-$VIF$(x, x')& $Otherwise  $
   \end{cases}
\]}
\label{def:visual_degrade}
\end{definition}

$\Delta_v$ returns a value between 0 and 1, with 0 indicating the no degradation to visual quality and 1 indicating all visual information in the original image has been changed. The first case of $\Delta_v$ corresponds to changes imperceptible to humans 
(when VSNR$(x, x')= \infty$) and changes that enhance the visual quality (when VIF$(x,x')>1$), indicating changes do not impact human recognition of the images negatively hence $\Delta_v = 0$. The other case deals with visible changes that degrade visual quality. Since VIF returns 1 for perfect quality compared to the original image, the degradation is one minus the image quality score. 

\noindent
\underline{Example:} In Fig.~\ref{fig:example}, the visual change of the original image Fig.~\ref{fig:a} is $0$ since no changes are applied, and Fig.~\ref{fig:b} has minimal frost added which caused minimal change in visual quality so $\Delta_v = 0.005$, and Fig.~\ref{fig:c} and Fig.~\ref{fig:d} have more frost and thus have higher $\Delta_v$ values $0.71$ and $0.96$.

\subsection{Measuring Human Recognition Robustness}
\label{sec:background_exp}
\red{TODO: a decision we need to make: do we do prediction preservation benchmark as well? }
The objective of the experiment with human participants, one per dataset, is to measure how human recognition performance is affected as changes in images, $\Delta_v$ value, increases. The design of the experiment is from Hu et al.~\cite{hu-et-al-22} following the experiment procedure by Geirhos et al.~\cite{Geirhos2018GeneralisationIH}. 

The experiment requires a transformation $T_X$; the dataset of original images $\{x_i\}$, $x_i\sim P_X$, with their ground-truth labels $\{f^*(x_i)\}$; and distributions $P_C$ for each transformation parameter. Then, a sample of transformed images $\{x_{i,j}’\}$, $x_{i,j}’\sim P_{T_X}$, is generated by randomly selecting $x_i$ from $\{x_i\}$ and $c_j\sim P_C$, and transforming $x_{i,j}’=T_X(x_i,c_j)$. The experiment to obtain human predictions for each image $\{x_{i,j}’\}$ is a \emph{forced-choice image categorisation task}: humans are presented with the images with transformations applied, for 200 ms, and asked to choose one of the given labels (e.g., car or bird)~\cite{Geirhos2018GeneralisationIH}. Since ILSRVR'12 dataset~\cite{ILSVRC2012} has 1,000 fine-grained classes and humans, when asked to label, can only categorize objects into entry-level classes (e.g. dog rather than German shepherd)~\cite{Geirhos2018GeneralisationIH}, humans are presented 16 entry-level class labels mapped by Geirhos et al.~\cite{Geirhos2018GeneralisationIH}: airplane, bicycle, boat, car, chair, dog, keyboard, oven, bear, bird, bottle, cat, clock, elephant, knife, truck. 
Between images, a noise mask is shown to minimize feedback influence in the brain~\cite{Geirhos2018GeneralisationIH}.
The tasks are timed to ensure fairness in the comparison between humans and machine~\cite{Firestone26562}. When sampling from $P_C$, it is ensured that the full range of achievable $\Delta_v$ values is covered~\cite{hu-et-al-22}. A given subject is never shown more than one version of an image $x_i$, whether original or transformed. 
%Note that human predictions for originals are different from their ground truth labels: labelers take as long as needed per image to classify it, but our subjects have only 200 ms to see each image.
%The human data is specific to a task, an image distribution, and a class of transformations, and thus has to be collected for the combination of the three. 

Data obtained this way is shown to be reusable for different samples from the same distribution, or, intuitively, for images sharing the same characteristics, e.g., the same image resolution, the same objects, etc.~\cite{hu-et-al-22}. %For example, it is reusable across different sets of images of road scenes taken within the same geographic area using cameras with same the resolution and image quality.

%\begin{itemize}
%    \item Visual Change (IQA definition and how it's used to get human performance)
%    \item What is Human Experiment?
%\end{itemize}
\red{TODO: Do we need how human data is plotted in background or in metrics?}

\red{I feel like this needs a section on its own after generating benchmarks.}

==> sections/benchmark_generation.tex <==
\section{Robustness Benchmark Generation} \label{section:benchmark-generation}
In this section, we formally define \robustness{} 
and describe the method for
%that our benchmark aims to check, and then the method for 
generating validation data. 
%\lm{It is not clear what existed and what is new.}
%{\bf MC:  test data or validation data? \purple{fixed}}
%then we present how test data are generated by our method. 

\noindent
\textbf{Background.} 
VCR considers average performance over visual change range. Performance is measured using a metric suitable for a given task. For image classification, we use accuracy and \emph{prediction similarity}~\cite{hu-et-al-22}. The latter measures the ability of a model to preserve its original prediction labels after applying transformations. In contrast to accuracy, it can be measured without ground truth, which is useful for robustness monitoring during deployment when no ground truth is available. We also use $\Delta_v$ to quantitatively measure the degree of visual change in the images for human observers~\cite{hu-et-al-22}. $\Delta_v$ is defined using an Image Quality Assessment metric called Visual Information Fidelity (\textit{VIF})~\cite{VIF, VIF_python}, which takes the original image $x$ and transformed image $x'$ as inputs and automatically predicts the human perceived image quality by measuring the perceptual ‘distance’ between the original and transformed images. Formally, $\Delta_v(x, x') = max(0, 1-\textit{VIF}(x, x'))$. To measure changes in image quality, 
%Using $\Delta_v$ while studying human robustness removes the complexity of different transformation parameter numbers and domains; and variance in the way an individual transformation is impacted by a particular transformation.  {\bf MC:  WHAT?}
%also how transformations can impact individual images differently. 
$\Delta_v$ returns a value between 0 and 1, with 0 indicating no degradation to visual quality and 1 indicating that all visual information in the original image has been changed. For example, the minimal blurring in Fig.~\ref{fig:a} caused a minimal change in visual quality of $\Delta_v = 0.02$, whereas the more pronounced blurring in Fig.~\ref{fig:b} corresponds to $\Delta_v = 0.94$.
See supplementary for more detail on $\Delta_v$.
%\lm{Why not mentioning that visual changes uses IQA, ML people would understand it, and it will look less magical.}\blue{\bf{[Addressed]}}
%\red{TODO: introduce with IQA, then say we define degradation as 1-IQA}
%\red{metric $(\Delta_v)$ based on IQA metric called VIF. VIF returns a value mostly between 0 and 1, can sometimes be $>1$ if the transformation increases image quality... representing a measure for image quality relative to the original image. $\Delta_v$ aims to represent degradation in the images, thus visual change is defined as $\Delta_v = max(0, 1-VIF)$.}

\noindent
\textbf{Definition of \robustness{}.}
We now define \robustness{} and distinguish it from existing robustness definitions.
% which generalizes  perturbation/corruption robustness~\cite{hendrycks2019robustness} and human-robustness changes~\cite{hu-et-al-22} to consider \emph{model} robustness \emph{against a wider and continuous range of realistic visual changes}. 
The \robustness{} is concerned with the average-case DNN performance over the entire range of $\Delta_v$ values a transformation can incur, with the maximum range being the $\Delta_v$ domain $[0,1]$. This range includes both small perturbations and big corruptions, as considered by perturbation robustness~\cite{hendrycks2019robustness} and corruption robustness~\cite{hendrycks2019robustness}. Additionally, this range also includes visual changes beyond those that do not affect human performance defined as model reliability~\cite{hu-et-al-22}.
%
% corruption robustness measures average-case performance on a given corruption, adversarial robustness measures the worst-case performance on small perturbations, perturbation robustness
%\red{TODO: add sentences clearly introducing existing definitions.}
%\red{Commonly used robustness include adversarial robustness; and also Perturbation robustness and corruption robustness which both came from~\cite{hendrycks2019robustness}. Compared to adversarial robustness and perturbation robustness, the main difference is that we consider a completely different and much larger range of changes. Compared to corruption robustness, our difference with them include 1) the range of changes we consider (uniformly sample VS 5 pre-selected); 2) we consider each transformation separately; 3) we also consider prediction similarity as used in~\cite{hu-et-al-22}. Compare to~\cite{hu-et-al-22}, which considers changes that do not affect human performance, we go beyond only not affecting human performance, and try to cover the full range of visual change values. }\blue{[Addressed below]}
%\blue{The concept of corruption robustness~\cite{hendrycks2019robustness} takes into account merely five pre-selected levels of severity, thereby failing to span the comprehensive $\Delta_v$ domain. Models evaluated on this basis could be susceptible against out-of-domain scenarios. Perturbation robustness~\cite{hendrycks2019robustness} and adversarial robustness considers even smaller perturbations that may be barely noticeable to humans. Our approach, \robustness{}, samples uniformly across the entire $\Delta_v$ domain, ensuring nearly complete coverage. We also incorporate prediction similarity~\cite{hu-et-al-22}, which can be used to measure the percentage of prediction labels that are not changed after applying corruptions. We go beyond the constraints of ~\cite{hu-et-al-22} which mainly targets changes that do not impact human performance by covering the full spectrum of $\Delta_v$.}
%
%Since visual change ($\Delta_v$) enables measuring human recognition performance for transformations with high dimensional parameter domains, we define \robustness{} using $\Delta_v$. Rather than focusing only on human-robustness changes as in \cite{hu-et-al-22} or pre-selected parameter values \purple{as corruption/perturbation robustness}~\cite{hendrycks2019robustness}, \robustness{} is concerned with the entire range of $\Delta_v$ values a transformation can incur, with the maximum range being the $\Delta_v$ domain $[0,1]$. This range includes both small perturbations and big corruptions. 
%
%For measuring model performance when changes are present, in addition to accuracy on the validation set measured by perturbation and corruption robustness, 
%Notice that \robustness{} considers \emph{average-case performance}, which is contrary to the worst-case performance considered by adversarial robustness.
We formally define \robustness{} as  follows:


\begin{definition}[\textbf{VCR ($\robustnesssymbol$)}]\label{def:visual-change-robustness}
Let a classifier $f$, a distribution of input images $P_X$, a ground-truth labeling function $f^*$, a transformation $T_X$ with parameter domain $C$,  % and parameter distribution $P_C$
and the visual change measure $\Delta_v$ be given. 
Given a $\Delta_v$ value $v \in [0,1]$, the \emph{joint distribution of original and transformed images with $v$} is $P(x,x'|v) = \frac{1}{P(v)}\int_C P(x’,v|x,c)P_X(x)P(c) dc$, where $x' =T_X(x, c)$, $v =\Delta_v(x, x')$ and $P(c)$ is uniform. %\red{TODO: not $c\in C$, since C is continuous, this should be an integral over c, which is $\int_C ... dc$}

%$P_{T_X, v}(x, x_i) = P_X(x)\sum_{c\in C, x_i=T_X(x, c), \Delta_v(x',x)=v} P_C(c)$. } \red{$P(x,x'|v)$, where x' ...}
%Define the full range of visual changes the transformation $T_X$ can incur as $V_d = \{\forall v_d \in [0, 1], s.t. v_d = \Delta_v(x_i, T_X(x_i, c))\}$ where $x_i \sim P_X, c\sim P_C$. }

\begin{subdefinition}[\textbf{VCR w.r.t. accuracy ($\robustnesssymbol_a$)}]\label{def:visual-change-robustness-acc}
Visual-change robustness of a classifier $f$ for accuracy is %$\mathbb{E}_{v \sim Uniform(0,1)}(P_{x, x_i \sim P_{TX, v}} (f(x_i) = f^*(x)))$. 
$\robustnesssymbol_a = \mathbb{E}_{v \sim \textit{Uniform(0,1)}}(P_{x, x'\sim P(x,x'|v)} (f(x') = f^*(x)))$.
\end{subdefinition}

\begin{subdefinition}[\textbf{VCR w.r.t. prediction similarity ($\robustnesssymbol_p$)}]\label{def:visual-change-robustness-pred-sim}
Visual-change robustness of a classifier $f$ for prediction similarity is %$\mathbb{E}_{v \sim Uniform(0,1)}(P_{x, x_i \sim P_{TX, v}} (f(x_i) = f(x)))$. 
$\robustnesssymbol_p = \mathbb{E}_{v \sim \textit{Uniform(0,1)}}(P_{x, x'\sim P(x,x'|v)} (f(x') = f(x)))$.
\end{subdefinition}
\label{def:robustness}
\end{definition}


%More specifically, in addition to using accuracy to judge 

%Let us assume that we are given an MVC $f$, a distribution of input images $P_X$, a ground-truth labeling function $f^*$, a transformation $T_X$ with parameter domain $C$ and parameter distribution $P_C$. Our requirements use the joint distribution of pairs of original and transformed images, defined as $P_{T_X}(x, x') = P_X(x)\sum_{c\in C, x'=T_X(x, c)} P_C(c)$.


%Define "range of changes" with delta v

%Modified versions of correctness and prediction properly defined, compared to common ML definitions.

%define prediction similarity

%\red{TO ADD: derivation to show sampling from X and C allows us to calculate this robustness}

%\red{definition 2, figure 4ab, how to plot should all be here to explain how we calculate these robustness definitions}

%\red{First we sample X and C, from this we generate a test set with x' = Tx(x, c) and v = Delta v(x, x'), we can obtain a sample set ? from $P(x, x', v, c)$. (Because we went from sampling from P(x) and P(c) to $P(x, x', v, c)$ since we obtained x' and v from x and c.)
%Then, separate ? into groups with same v value (in practice we use small intervals) -> sample to calculate $P(x, x'|v)$ this is because we aggregate different c values. 
%For each v value from 0 to 1, we calculate $P_{x, x'\sim P(x,x'|v)} (f(x') = f^*(x))$ (accuracy) and pred sim (percentage of the same labels).
%Then we put these into a plot we obtain 4a and 4b depending on whether it's human or ML. To find expectation of v in [0, 1], we do area under the curve integral. (definition 2)
%}

\noindent
\textbf{Validation Set Generation.} 
To measure \robustness{} of humans or DNNs, our method \method{} generates a validation set (Step~\RN{1} of Fig.~\ref{fig:intro-paper-design-flowchart}) for a given transformation $T_X$. First, we sample $x\sim P_X$ and $c \sim \textit{Uniform}(C)$, and obtain $x'=T_X(x, c)$ and $v= \Delta_v(x, x')$, resulting in samples $(x, x', c, v)$. % We divide a continuous parameter domain $C$ into $M$ random levels for sampling.
Next, we divide them into groups of $(x,x’,c)$, each with the same $v$ value. %Thus, the resulting groups are samples from $P(x,x’,c|v)$.
Finally, by dropping $c$, we obtain groups of $(x,x’)$ with the same $v$, which are samples from $P(x,x’|v)$. 

Then, to measure $\robustnesssymbol_a$ [resp. $\robustnesssymbol_p$] of a subject (a human or a DNN) for each $v$ value sampled, we calculate $a_v = P_{x, x'\sim P(x,x'|v)} (f(x') = f^*(x))$ [resp. $p_v = P_{x, x'\sim P(x,x'|v)} (f(x') = f(x))$] with our $(x, x')$ samples. By plotting $v,a_v$ [resp. $v, p_v$] and applying monotonic smoothing splines~\cite{koenker-94} to reduce randomness and outliers, we obtain spline curves $s_a$ [resp. $s_p$]. The spline curves represent how human performance decreases as we increase visual change in images. For example, the curve $s^h_a$ for human accuracy is shown in Fig.~\ref{fig:metric-human-performance-integral}, whereas the one for DNN $s^m_a$ is shown in Fig.~\ref{fig:metric-ml-performance-integral}. %\red{TODO: monotonically decreasing curve, + a figure for demonstration of smoothing}

Finally, we estimate $\robustnesssymbol_a = \mathbb{E}_{v \sim \textit{Uniform(0,1)}}(a_v)$ [resp. $\robustnesssymbol_p =\mathbb{E}_{v \sim \textit{Uniform(0,1)}}(p_v)$] as the area under the spline $s$, i.e., $\hat{\robustnesssymbol}_a = A_a = \int_0^{1} s_a(v) dv$ [resp. $\hat{\robustnesssymbol}_p =A_p = \int_0^{1} s_p(v) dv$]. In Fig.~\ref{fig:metric-human-performance-integral}, the area $A^h_a$ used to calculate human $\robustnesssymbol_a$ is highlighted in yellow; and in Fig.~\ref{fig:metric-ml-performance-integral}, $A^m_a$ for calculating DNN model $\robustnesssymbol_a$ is highlighted in blue.

\noindent
\textbf{Benchmark Generated.}
The validation dataset created for a specific transformation  encompasses 50,000 images, mirroring the size of the \textsc{ImageNet}~\cite{ILSVRC2012} validation set. These constructed datasets essentially span the full spectrum of $\Delta_v$,  unlike \imagenetc~\cite{hendrycks2019robustness}, which covers it only  partially. See the supplementary for the $\Delta_v$ distribution plots. For experiments in this paper, we considered 14 different image transformations: Shot Noise, Impulse Noise, Gaussian Noise, Glass blur, Gaussian Blur, Defocus Blur, Motion Blur, Brightness and Frost from \imagenetc~\cite{hendrycks2019robustness}; Blur, Median Blur, Hue Saturation Value and Color Jitter from Albumentations~\cite{albumentation}; and Uniform Noise from Gehiros et. al~\cite{Geirhos2018GeneralisationIH}. See supplementary for a demonstration of these transformations.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{resources/metric/metrics.png}
%     \caption{Metrics comparing a given model with human performance for a given transformation}
%     \label{fig:metrics-illustration}
% \end{figure}

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.95\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/metric-big-legend.png}
         \label{fig:metric-illustration-legend}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/human-integral.png}
         \caption{\scriptsize Human Performance}
         \label{fig:metric-human-performance-integral}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/ml-integral.png}
         \caption{\scriptsize Model Performance}
         \label{fig:metric-ml-performance-integral}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/human-completely-better-than-ml.png}
         \caption{\scriptsize Human More Robust}
         \label{fig:metric-human-better-ml}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/ml-completely-better-than-human.png}
         \caption{\scriptsize DNN More Robust}
         \label{fig:metric-ml-better-huamn}
     \end{subfigure}
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/metric/human-ml-diff.png}
         \caption{\scriptsize DNN vs Human}
         \label{fig:metric-human-ml-difference}
     \end{subfigure}
     
    \caption{\robustness{} comparison of a DNN with human performance for a given transformation through comparison of estimated spline curves.}
    \label{fig:metric-curve}
    \vspace{-0.15in}
\end{figure}


%A validation set $\{x_{i,j}'\}$ for a transformation $T_X$ should consist of transformed images with $\Delta_v$ scores that is a fair sample of the entire range of $\Delta_v$ scores, i.e., $V_d$.  
%Our framework, given a transformation $T_X$ with parameter domain $C$ with distribution $P_C$ and a dataset $\{x_i\}$ where $x_i \sim P_X$, generates a validation set $\{x_{i, j}'\}$. First, $M$ sets of parameter values $\{c_j\}$ are sampled from $C$ where $c_j \sim P_C$. Using $\{c_j\}$ rather than a fixed number of pre-selected parameter values would result in images that cover more possible values of $\Delta_v$.  
%Then for each $\{c_j\}$, $N$ original images $x_i$ are sampled from $\{x_i\}$. For each pair of $(x_i, c_j)$ a test image is created by $x_{i,j}' = T_X(x, c_j)$. As a result, a validation set $\{x_{i, j}'\}$ of size $M\times N$ is created. 


%\purple{Generating images by sampling from the parameter domain to cover the widest possible range of changes we can reach, we use 'uniform' sampling. This also guarantees the variaty of combination of parameter values for different visual change scores. }
%Given the visual change metric $\Delta_v$, \robustness{} focuses on whether the performance of $f$ is affected by a specific range of visual change that can by introduced by applying $T_X$, that is $\Delta_v$ between $0$ and $1$ or the maximum $T_X$ can achieve if less than $1$. 
%To test \robustness{} for the full range of visual change introduced by applying a transformation $T_X$, the test sequence $\{x_{i, j}'\}$ should cover test images that have different $\Delta_v$ values between $0$ and $1$; or if $1$ is not achievable, between $0$ and the maximum $\Delta_v$ value the transformations can achieve. 

%Given a image dataset, a sample size n and a transformation type, n images are randomly sampled from the given dataset, and the transformation parameter is randomly sampled. We divided each transformation into 1000 levels and the transformation parameter is randomly chosen from the 1000 levels. The goal of this uniform random parameter selection is to cover the visual change range. Which is the x axis in Figure ?. The larger the sample size, the more precise the benchmark will be.
%\purple{The range of changes considered by \robustness{} include both small perturbation and big corruptions, regardless of whether humans are robust to the changes. Contrary to adversarial robustness, which measures the worst-case performance facing a perturbation, \robustness{} considers average-case performance facing the entire range of changes that $T_X$ can incur. }
%For measuring ML performance, in addition to accuracy on test sequence measured by perturbation and corruption robustness, \robustness{} also considers the percentage of prediction labels that are not changed after applying $T_X$, called prediction similarity~\cite{hu-et-al-22}. Prediction similarity can be measured without ground truth, which is useful for robustness monitoring during deployment when no ground truth is available~\cite{hu-et-al-22}. 
%\noindent
%\underline{Example:} In Fig.~\ref{fig:example}, the visual change of the original image Fig.~\ref{fig:a} is $0$ since no changes are applied, and Fig.~\ref{fig:b} has minimal frost added which caused minimal change in visual quality so $\Delta_v = 0.005$, and Fig.~\ref{fig:c} and Fig.~\ref{fig:d} have more frost and thus have higher $\Delta_v$ values $0.71$ and $0.96$.

%\red{TO ADD: Imagnet-c considers a corruption as a pair of transformation and a selected parameter value, while we consider a transformation and its entire parameter domain.}

==> sections/checklist.tex <==
\section{Checklist}

%The NeurIPS Paper Checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. For each question in the checklist:

%You should answer yes, no, or n/a.
%You should reference the section(s) of the paper that provide support for your answer.
%You can also optionally write a short (1–2 sentence) justification of your answer.
%You are encouraged to take a look at the checklist early on as it likely will positively influence the way you do your research and write the paper, rather than treating it as an afterthought.

%Reviewers will be asked to use the checklist as one of the factors in their evaluation. The questions are mostly framed in terms of transparency: "Did you include [information]?" While "yes" is generally preferable to "no", it is perfectly acceptable to answer "no" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "no" or "n/a" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgement and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material.

%We provide guidance on how to answer each question below. You may additionally refer to the blog post from 2021 introducing the checklist to learn more about its motivation and how it was created.

For all authors...

(a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \red{yes}

%Claims in the paper should match theoretical and experimental results in terms of how much the results can be expected to generalize.

%The paper's contributions should be clearly stated in the abstract and introduction, along with any important assumptions and limitations. It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.

(b) Have you read the ethics review guidelines and ensured that your paper conforms to them?  \red{yes}

%Please read the ethics review guidelines.

(c) Did you discuss any potential negative societal impacts of your work?  \red{yes}

%Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), environmental impact (e.g., training huge models), fairness considerations (e.g., deployment of technologies that could further disadvantage historically disadvantaged groups), privacy considerations (e.g., a paper on model/data stealing), and security considerations (e.g., adversarial attacks).

%We expect many papers to be foundational research and not tied to particular applications, let alone deployments, but being foundational does not imply that research has no societal impacts. If you see a direct path to any negative applications, you should point it out, even if it's not specific to your work. In a theoretical paper on algorithmic fairness, you might caution against overreliance on mathematical metrics for quantifying fairness and examples of ways this can go wrong. If you improve the quality of generative models, you might point out that your approach can be used to generate Deepfakes for disinformation. On the other hand, if you develop a generic algorithm for optimizing neural networks, you do not need to mention that this could enable people to train models that generate Deepfakes faster.

%Consider different stakeholders that could be impacted by your work. It is possible that research benefits some stakeholders while harming others. Pay special attention to vulnerable or marginalized communities.

%Consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.

%If there are negative societal impacts, you should also discuss any mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).

%For more information, see this unofficial guidance from last year and other resources at the broader impacts workshop at NeurIPS 2020.

(d) Did you describe the limitations of your work? \red{yes}

%You are encouraged to create a separate "Limitations" section in your paper.

%Point out any strong assumptions and how robust your results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). Reflect on how these assumptions might be violated in practice and what the implications would be.

%Reflect on the scope of your claims, e.g., if you only tested your approach on a few datasets or did a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.

%Reflect on the factors that influence the performance of your approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be able to be reliably used to provide closed captions for online lectures because it fails to handle technical jargon.

%We understand that authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection. It is worth keeping in mind that a worse outcome might be if reviewers discover limitations that aren't acknowledged in the paper. In general, we advise authors to use their best judgement and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.

%For more guidance, please refer to this 2022 FAccT paper by Smith, et al.

If you are including theoretical results...

(a) Did you state the full set of assumptions of all theoretical results? \red{yes}

%All assumptions should be clearly stated or referenced in the statement of any theorems.

(b) Did you include complete proofs of all theoretical results? \red{yes}

%The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, authors are encouraged to provide a short proof sketch to provide intuition.

%You are encouraged to discuss the relationship between your results and related results in the literature. 

If you ran experiments...

(a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \red{yes}

%The instructions should contain the exact command and environment needed to run to reproduce the results.

%Please see the NeurIPS code and data submission guidelines for more details.

%Main experimental results include your new method and baselines. You should try to capture as many of the minor experiments in the paper as possible. If a subset of experiments are reproducible, you should state which ones are.

%While we encourage release of code and data, we understand that this might not be possible, so "no because the code is proprietary" is an acceptable answer.

%At submission time, to preserve anonymity, remember to release anonymized versions.

(b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? \red{yes}

%The full details can be provided with the code, but the important details should be in the main paper.

(c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \red{yes}

%Answer "yes" if you report error bars, confidence intervals, or statistical significance tests for your main experiments.

(d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \red{yes}

%Ideally, you would provide the compute required for each of the individual experimental runs as well as the total compute.

%Note that your full research project might have required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). The total compute used may be harder to characterize, but if you can do that, that would be even better.

%You are also encouraged to use a CO2 emissions tracker and provide that information. See, for example, the experiment impact tracker (Henderson et al.), the ML CO2 impact calculator (Lacoste et al.), and CodeCarbon.

%If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...

(a) If your work uses existing assets, did you cite the creators? \red{yes}

%Cite the original paper that produced the code package or dataset.

%Remember to state which version of the asset you're using.

%If possible, include a URL.

(b) Did you mention the license of the assets? \red{yes}

%State the name of the license (e.g., CC-BY 4.0) for each asset.

%If you scraped data from a particular source (e.g., website), you should state the copyright and terms of service of that source.

%If you are releasing assets, you should include a license, copyright information, and terms of use in the package. If you are using a popular dataset, please check paperswithcode.com/datasets, which has curated licenses for some datasets. You are also encouraged to use their licensing guide to help determine the license of a dataset.

%If you are repackaging an existing dataset, you should state the original license as well as the one for the derived asset (if it has changed).

%If you cannot find this information online, you are encouraged to reach out to the asset's creators.

(c) Did you include any new assets either in the supplemental material or as a URL? \red{yes}

%During submission time, remember to anonymize your assets. You can either create an anonymized URL or include an anonymized zip file.

%If you cannot release (e.g., the asset contains proprietary information), state the reason.

(d) Did you discuss whether and how consent was obtained from people whose data you're using/curating? \red{yes  }

%For example, if you collected data from via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?

%Even if you used an existing dataset, you should check how data was collected and whether consent was obtained. We acknowledge this might be difficult, so please try your best; the goal is to raise awareness of possible issues that might be ingrained in our community.

(e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? \red{n/a, only classification labels are collected.}

%There are some settings where the existence of this information is not necessarily bad (e.g., swear words occur naturally in text). This question is just to encourage discussion of potentially undesirable properties.

%Explain how you checked this (e.g., with a script, manually on a sample, etc.).

%If you used crowdsourcing or conducted research with human subjects...

(a) Did you include the full text of instructions given to participants and screenshots, if applicable? \red{yes}

%Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.

(b) Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \red{n/a, no potential risk}

%Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.

%Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.  For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review.

(c) Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation? \red{yes}

%First, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take.
%Also include discussion on how the wage was determined and how you determined that this was a fair wage.

==> sections/eval_metrics.tex <==
\section{Human-Aware Evaluation Metrics} \label{sec:eval-metrics}
%\red{Eval metrics to compare this robustness with human, Ah/Ah-m}
After generating a validation set (Step~\RN{1}) and collecting human performance data (Step~\RN{2}) for our method {\method} (as depicted in Fig.~\ref{fig:intro-paper-design-flowchart}), we now evaluate the performance of DNNs by comparing it to human performance (Step~\RN{3}).
%\lm{The story here misses connections pieces.}\red{[Addressed]}
%To compare DNN model \blue{\robustness{}} to a human, we aim to evaluate DNN performance relative to a human performance.
%To measure the reliability of a DNN model compared to a human, we want to evaluate DNN performance in relation to human performance.



Using human robustness data collected in Step 2 (Fig.~\ref{fig:intro-paper-design-flowchart})  and DNN predictions, we first obtain the following spline curves: for $\robustnesssymbol_a$, 1) $s^h_a$ for humans and 2) $s^m_a$ for the DNN, see Fig.~\ref{fig:metric-human-better-ml}-\ref{fig:metric-human-ml-difference};  similarly for $\robustnesssymbol_p$, 1) $s^h_p$ for humans and 2) $s^m_p$ for the DNN. 

We then use two new
%In this section, we propose our new 
human-aware evaluation metrics  \emph{Human-Relative Model Robustness Index} (\emph{HMRI}) and  \emph{Model Robustness Superiority Index} (\emph{MRSI}). %that takes human performance into account and measures how DNN robustness is proportional to human performance.
% Definition starts here
\begin{definition}[\textbf{Human-Relative Model Robustness Index (\textit{HMRI})}]
%Checks how much human performance DNN models can achieve.\\
Given spline curves $s^h$ and $s^m$, let $A_{h>m} = \int_0^{1}(s^h(v)-s^m(v))^+ dv$ denote the average (accuracy or preservation) performance lead of a human over a model across the visual change range, where the performance lead is defined as the positive part of performance difference, i.e., $(s^h(v)-s^m(v))^+=max(0,s^h(v)-s^m(v))$. The Human-Relative Model Robustness Index (\textit{HMRI}), which quantifies the extent to which a DNN can replicate human performance, is defined as $\textit{HMRI}=\frac{A_{h}-A_{h>m}}{A_h}=1-\frac{A_{h>m}}{A_h}$.
\label{def:metric-HMRI}
\end{definition}

\begin{definition}[\textbf{Model Robustness Superiority Index (\textit{MRSI})}]
%Checks how much DNN can exceed human.\\
Given spline curves $s^h$ and $s^m$, let $A_{m>h} = \int_0^{1}(s^m(v)-s^h(v))^+ dv$ denote the average performance lead of a model over a human across the visual change range. The Model Robustness Superiority Index (\textit{MRSI}), which quantifies the extent to which a DNN model can surpass human performance, is defined as $\textit{MRSI}=\frac{A_{m>h}}{A_m}$.
\label{def:metric-MRSI}
\end{definition}

Comparing humans and DNNs with \textit{HMRI} and \textit{MRSI}  yields three possible scenarios shown in Fig.~\ref{fig:metric-human-better-ml}-\ref{fig:metric-human-ml-difference}: (1)  human performance fully exceeds DNN's, i.e., $0<\textit{HMRI}<1$ and $\textit{MRSI}=0$, see Fig.~\ref{fig:metric-human-better-ml}; (2)  DNN's performance fully exceeds humans', i.e., $\textit{HMRI}=1$ and $\textit{MRSI} > 0$, see Fig.~\ref{fig:metric-ml-better-huamn}; and (3)  human performance is better than DNN's in some $\Delta_v$ intervals and worse in others, i.e., $\textit{HMRI} < 1$ and $\textit{MRSI} > 0$, see Fig.~\ref{fig:metric-human-ml-difference}.


% In Figure \ref{fig:metric-human-ml-difference}, HMRI is represented as the ratio of the green region to the combined green and yellow region. Similarly, MRSI is depicted as the ratio of the blue region to the combined blue and yellow region.

\textit{HMRI} takes both DNN and human performance into the equation. As shown in Fig.~\ref{fig:metric-human-better-ml} and Fig.~\ref{fig:metric-human-ml-difference}, $A_{h>m}$, highlighted in yellow, represents the area where human performance is better than DNN; and $A_{h}-A_{h>m}$, highlighted in green, represents %the \blue{percentage} 
the area where the DNN can be comparable to human performance.
%\blue{how much human performance the DNN can be comparable with. }%of human performance that the DNN can reach. Thus, 
\textit{HMRI} is calculated as the green region over the entire $A_h$ (combined green and yellow region), which is $\frac{A_{h}-A_{h>m}}{A_h}$. 
The \textit{HMRI} value ranges from $[0,1]$; a higher \textit{HMRI} indicates a DNN model closer to human \robustness{}, and $\textit{HMRI}=1$ signifies that $s^m$ is the same as or completely above $s^h$ in the entire $\Delta_v$ domain, meaning that the DNN is at least as reliable as a human.

% \red{update to match the new $M_{m>h}$.}
% \red{It is possible that ...}
\emph{Corruption Error (CE)} is a metric defined in \imagenetc~\cite{hendrycks2019robustness} as the top-1 classification error rates on the corrupted images, normalized by the error rates of a baseline model. We can compare a DNN with a human if the baseline model is set to be human. However, CE is not able to determine whether a DNN can exceed a human in some cases (Fig.~\ref{fig:metric-human-ml-difference}).
%incapable of indicating whether a DNN can exceed human.}
DNN models could potentially have super-human accuracy for particular types of perturbations or in some $\Delta_v$ ranges.  Thus we also want to measure how much a DNN can \emph{exceed} human performance. As shown in  Fig.~\ref{fig:metric-human-ml-difference}, $A_{m>h}$, highlighted in blue, represents the area where DNN performance exceeds a human; and $A_{m}-A_{m>h}$, highlighted in green (equal to $A_{h}-A_{h>m}$), represents human performance that the DNN can reach. \red{here is motivation}
%also can be interpreted as the area under the ML performance curve $m$ such that DNN does not exceed humans. 
Thus, \textit{MRSI} is calculated as the green area over the entire $A_m$ (combined green and blue regions), which is $\frac{A_{m}-A_{m>h}}{A_m}$. %Intuitively, $P_{h-m}$ measures how much DNN models can outperform humans. 
The \textit{MSRI} value ranges from $[0,1)$, with the higher value indicating better performance than humans. $\textit{MSRI}=0$ means that the given DNN model performs worse than or equal to human in the entire $\Delta_v$ domain. A positive \textit{MSRI} value indicates that the given DNN model performs better than human at least in some ranges of $\Delta_v$.

For example, as shown in Fig.~\ref{fig:metric-curve}, Fig.~\ref{fig:metric-human-better-ml} (human always performs better) would yield $\textit{HMRI}\in[0,1)$ and $\textit{MRSI}=0$; Fig.~\ref{fig:metric-ml-better-huamn} (DNN always performs better) would yield $\textit{HMRI}=1$ and $\textit{MRSI}\in (0,1)$; Fig.~\ref{fig:metric-human-ml-difference} (DNN and human outperform each other in different $\Delta_v$) would yield $\textit{HMRI}\in(0,1)$ and $\textit{MRSI}\in(0,1)$.



% ==================
% Below is old metric section



% \red{As shown in step~\RN{3} of Fig.~\ref{fig:intro-paper-design-flowchart}, we evaluate DNN \robustness{} on our generated validation set with respect to human performance. Given any transformation, after steps~\RN{1} and~\RN{2}, we obtained .... the splines, then we want to compare.... }
\begin{comment}
    

\blue{
As shown in Step~\RN{2} of Fig.~\ref{fig:intro-paper-design-flowchart}, we evaluate DNN \robustness{} on our generated validation set with respect to human performance. Given any transformation, we can obtain evaluation results for DNN performance and human performance after Steps~\RN{1} and~\RN{2}.}

\red{TODO: compare with mCE, this metric does not indicate whether ML can exceed humans ... they also do percentage of one compared  to another}

%By doing a set of experiments with humans and a ML model, data points can be grouped into accuracy bins based on $\Delta_v$.
{\bf MC:  I feel that this section skipped a few steps}
Using human robustness data {\bf MC:  where is it collected?} and DNN predictions, we first obtain the following spline curves: for $\robustnesssymbol_a$, 1) $sp^h_a$ for humans and 2) $sp^m_a$ for the DNN, see Fig.~\ref{fig:metrics-illustration}c-\ref{fig:metrics-illustration}e; then similarly for $\robustnesssymbol_p$, 1) $sp^h_p$ for humans and 2) $sp^m_p$ for the DNN. 

Comparing humans and DNNs \blue{with $\robustnesssymbol_a$} {\bf MC:  w.r.t. which metric?} yields three possible scenarios. \blue{To account for them, we define two metrics for comparing DNN performance with human performance: 1) Human Model Robustness Index (HMRI), 2) Model Robustness Superiority Index (MRSI). }

% that one measures the percentage of human performance a DNN model can achieve and second how much a given DNN model can exceed humans.}
% \blue{shown in Fig.~\ref{fig:metrics-illustration}c-~\ref{fig:metrics-illustration}e.  }

\blue{We define 2 metrics for comparing DNN performance with human performance: 1) Human Model Robustness Index (HMRI), 2) Model Robustness Superiority Index (MRSI).}

\red{how to describe the two measures in English: 1) Human model robustness index (HMRI), 2) model robustness Superiority index (MRSI)}

\red{all given XXX should be the spline models}

shown in Fig.~\ref{fig:metrics-illustration}c-~\ref{fig:metrics-illustration}e: (1) when human performance fully exceeds DNN's, i.e., $M_h<1$ and $M_{m>h}=0$, see Fig,~\ref{fig:metric-human-better-ml}; (2) when DNN's perormance fully exceeds humans', i.e., $M_h=1$ and $M_{m>h} > 0$, see Fig.~\ref{fig:metric-ml-better-huamn}; and (3) when human peformance is better than DNN's in some $\Delta_v$ intervals and worse in others, i.e., $M_h < 1$ and $M_{m>h} > 0$, see
 Fig.~\ref{fig:metric-human-ml-difference},  \red{remove the mentions of M here}
 {\bf MC : I have rewritten this paragraph.  Please check for correctness}

%As shown in Fig.~\ref{fig:metric-human-better-ml}-\ref{fig:metric-human-ml-difference}, when comparing human and DNN, there are three possible scenarios, 1) Human completely exceeds DNN, Fig.~\ref{fig:metric-human-better-ml}; 2) DNN completely exceeds human, Fig.~\ref{fig:metric-ml-better-huamn}; 3) Human and DNN exceed each other in different $\Delta_v$ intervals, Fig.~\ref{fig:metric-human-ml-difference}. Therefore, to account for these scenarios, .}
%and $P_{m-h}$ to measure the proportion of human performance a DNN model can achieve and how much a DNN model can exceed human performance respectively. 
Given a pair of spline curves $sp^h_a$ and $sp^m_a$, or $sp^h_p$ and $sp^m_p$, we define two metrics for measuring DNN \robustness{} compared to humans: 1) $M_{h}$, which measures the proportion {\bf MC:  again, I am not sure why we are measuring proportions?} of human performance a DNN model can achieve; and 2) $M_{m>h}$, which is how much a DNN model can exceed human performance.  {\bf MC:  why are these the right metrics?  why are they useful?} \red{$<-$ to cover the scenarios}
%Using $A_h$ and $A_m$, 

\begin{definition}
%Checks how much human performance DNN models can achieve.\\
Given XXX, let $A_{h>m} = \int_0^{1}sp^h(v)-min(sp^m(v), sp^h(v)) dv$ denote  the amount of performance surplus human has on DNN model regarding accuracy.  {\bf MC:  WHAT? } \red{should be green over all yellow} 
Therefore, $M_{h}$ measuring the relative performance of a DNN model comparing to a human (i.e., how much human performance DNN can achieve), is defined as:
$M_{h}=\frac{A_{h}-A_{h>m}}{A_h}=1-\frac{A_{h>m}}{A_h}$.
\label{def:metric-h-m}
\end{definition}

%$A_m$ doesn't involve comparison with human. 
$M_{h}$ takes both DNN and human performance into the equation. As shown in Fig.~\ref{fig:metric-human-better-ml} and Fig.~\ref{fig:metric-human-ml-difference}, $A_{h>m}$, highlighted in yellow, represents the area where human performance is better than DNN; and $A_{h}-A_{h>m}$, highlighted in green, represents the amount  {\bf MC:  we cannot measure human performance in amounts!}\red{percentage} of human performance that the DNN can reach. Thus, 
%area under the human performance spline $sp^h$ such that DNN performs better than a human. 
$M_{h}$ is calculated as a green area over the entire $A_h$, which is $\frac{A_{h}-A_{h>m}}{A_h}$. %We can interpret $M_{h>m}$ as how much human performance can an DNN model reach.
%See Fig. \ref{fig:metric-human-ml-difference} for a visualization of $A_{h-m}$.
The $M_h$ value ranges from $[0,1]$; a higher $M_h$ indicates a DNN model closer to human \robustness{}, and $M_h=1$ signifies that $sp^m$ is the same as or completely above $sp^h$, meaning the DNN is at least as reliable as a human.


\begin{definition}
%Checks how much DNN can exceed human.\\
We denote the amount of performance surplus DNN has on humans {\bf MC: 
 again, I have a problem with the term} \red{how much ML can exceed humans} as $A_{m>h} = \int_0^{1}sp^m(v)-min(sp^m(v), sp^h(v)) dv$. Therefore, $M_{m>h}$ measuring how much DNN can outperform humans is 
%We use $M_{m>h}$ to denote the relative performance of human comparing to an DNN model.% (i.e. \purple{how much DNN can outperform humans}).
%$M_{m>h}=\frac{A_{m}-A_{m>h}}{A_m}=1-\frac{A_{m>h}}{A_m}$.
$M_{m>h}=\frac{A_{m>h}}{A_m}$.
\label{def:metric-m-h}
\end{definition}

%it can cover the entire human performance area (i.e. at least as reliable as human), and less than 1 if the accuracy at some visual change cannot reach human level. 
\red{update to match the new $M_{m>h}$.}
\red{It is possible that ...}DNN models can have super-human accuracy for particular types of perturbations. {\bf MC:  which ones?} Thus we also want to measure how much DNN can \emph{exceed} human performance. As shown in  Fig.~\ref{fig:metric-human-ml-difference}, $A_{m>h}$, highlighted in blue, represents the area where DNN performance exceeds a human; and $A_{m}-A_{h>m}$, highlighted in green, is the same as $A_{h}-A_{h>m}$ representing human performance that the DNN can reach.
%also can be interpreted as the area under the ML performance curve $m$ such that DNN does not exceed humans. 
Thus $M_{m>h}$ is calculated as the green area over the entire $A_m$, which is $\frac{A_{m}-A_{m>h}}{A_m}$. %Intuitively, $P_{h-m}$ measures how much DNN models can outperform humans. 
The $M_{m>h}$ value ranges from $[0,1)$, with the higher value indicating better performance than humans.  

\red{For example, as shown in Fig.~\ref{fig:metric-curve}, in the three senarios, which scenario would result in what M value. },
\end{comment}
%1) Human completely exceeds DNN, Fig.~\ref{fig:metric-human-better-ml}; 2) DNN completely exceeds human, Fig.~\ref{fig:metric-ml-better-huamn}; 3) Human and DNN exceed each other in different $\Delta_v$ intervals, Fig.~\ref{fig:metric-human-ml-difference}. For 1) 

%In the scenario of Fig.~\ref{fig:metric-human-ml-difference}, where DNN exceeds human when $\Delta_v$ is low and human exceeds DNN when $\Delta_v$ is large, $P_{h-m}\in (0, 1)$, $P_{m-h}\in (0, 1)$. Additionally, there are two special cases for the metrics. As shown in Fig.~\ref{fig:metric-ml-better-huamn}, when DNN completely exceeds human performance, $P_{h-m}=0$ and $P_{m-h}\in[0, 1)$. As shown in Fig.~\ref{fig:metric-human-better-ml}, when human completely exceeds DNN performance, $P_{m-h}=0$ and $P_{h-m}\in[0, 1)$. \\



% \red{TODO: illustrate the two definitions using the pictures you created. If a model looks like this, what is the value of the two metrics, what can we learn about this model. Maybe we can create some more pictures where ML is completely better than humans, one where it is completely worse to illustrate the metrics.}\\

% \red{TODO: this is good, move them up, see my comments in the definition. Only leave the comparison between h-m and m-h here}


% However $A_{human-ml}$ is an absolute difference between human and ML model, which has different meanings when $A_{human}$ has different values.\\
% Thus we define new metric $D_{ml-human}=\frac{A_{human-ml}}{A_{human}}$ which is a metric in percentage. \\
% The value goes to zero when $A_{human-ml}$ goes to zero, which means, human is no better than the ML model being evaluated in the entire visual range.\\
% On the contrary, $D_{ml}=\frac{A_{ml-human}}{A_{human}}$ represents how much the ML model is ahead of human in percentage. This value is expected to be as high as possible.


% \begin{definition}
% Let an image $x$, an applicable transformation $T_X$ with a parameter domain $C$ and a parameter $c\in C$, s.t. $x' = T_X(x,c)$ be given.
% Visual change $\Delta_v(x,x')$ is a function defined as follows:
%     {\small  \[ \begin{cases} 
%       0  & $If VSNR$(x, x')= \infty \\
%       &$ or VIF$(x,x')>1\\
%        1-$VIF$(x, x')& $Otherwise  $
%    \end{cases}
% \]}
% \label{def:visual_degrade}
% \end{definition}


% \noindent- How is a curve defined and plotted?\\
%     \indent\quad- Based on human performance data\\
% - How is the new metric defined?\\
%     \indent\quad- With area under performance curve\\
%     \indent\quad- Percentage (difference over human area)\\
% - How to handle edge cases?\\
%     \indent\quad- What if positive and negative integral differences cancel each other out and result in 0 difference?\\

%and $sp^h_p$ for $\robustnesssymbol_p$. After checking DNN model predictions on the validation set, we obtain for DNN model performance $sp^m_a$ for $\robustnesssymbol_a$ and $sp^m_p$ for for $\robustnesssymbol_p$. As shown in Fig.~\ref{fig:metric-human-better-ml}, Fig.~\ref{fig:metric-ml-better-huamn} and Fig.~\ref{fig:metric-human-ml-difference}. }

%\red{TODO: match definitions below with new definition and notation}%In the later definitions of this section, each performance metric has 2 versions, one regarding accuracy and one regarding prediction similarity. They are distinguished with superscript, $a$ for accuracy and $p$ for prediction similarity. They are exactly the same in nature except one measures performance regarding accuracy and another measures performance regarding prediction similarity. So we only explicitly provide the definition of the accuracy version. 
%For example, for a transformation \red{temp?} $h_a$ and $m_a$ using model \red{temp?} are shown in Fig.~\ref{fig:metric-human-performance-integral}.
%We can obtain two accuracy curves after sorting the accuracy bins against $\Delta_v$ where the $x$-axis is $\Delta_v$ and the $y$-axis is accuracy at the corresponding $\Delta_v$. 
%We call them human performance curve and ML performance curve, denoted by $h(v)$ and $m(v)$. See definition \ref{def:metric} for the definition of our evaluation metric.

\begin{comment}

\begin{definition}
%Let $x\sim P_X, c\sim P_C, x'=T_X(x, c)$. Let $v$ be $\Delta_v(x,x')$, i.e. the visual change between the original and the transformed image. 
\red{duplicated} Given a pair of spline models $h$ and $m$ ($h_a$ and $m_a$ for correctness or $h_p$ and $m_p$ for prediction similarity), we denote the area ($A$) under the curve $h$ as $A_h$ and under $m$ as $A_m$ respectively:
%the performance of human and DNN model regarding accuracy with $A^a_h$ and $A^a_m$ respectively; and the performance of human and DNN model regarding prediction similarity with $A^p_h$ and $A^p_m$ respectively, where $A$ stands for the area under the performance curve. They are defined as
\begin{align*}
A_{h} &= \int^1_0 h(v) dv \\
A_{m} &= \int^1_0 m(v) dv
\end{align*}
\end{definition}

\purple{In Fig. \ref{fig:metric-human-performance-integral}, the orange curve is $h_a$ which represents how human accuracy changes as $\Delta_v$ value changes, therefore  x-axis is $\Delta_v$ value and y-axis is accuracy. The range of both x- and y-axis are $[0,1]$. The area under $h_a$, highlighted in yellow, is $A_h$. Similarly in Fig.~\ref{fig:metric-ml-performance-integral}, $m_a$ is shown as the blue curve and $A_m$ is the area under $m_a$ highlighted in blue. }
We use area under the performance curve to define performance because we are measuring robustness and we expect the accuracy at any level of visual change to be as high as possible. If a DNN model can reach 100\% at any level of visual change, then the performance $A_m$ will be 1.

\end{comment}


==> sections/evaluation.tex <==
% Evaluation Section Content: experimental setup, the metrics used, the results obtained, and the implications of the findings
\section{Evaluation}
\label{sec:evaluation}

In this section, we present experiments evaluating our proposed method \method.
First, we verify that human robustness data can be reused for similar transformations.  Second, we present results on comparing to humans the robustness of the DNNs that are top-performing on the \SoTA{} image corruption benchmark dataset \imagenetc~\cite{hendrycks2019robustness}. 
Finally,   we train the models on the {\method} transformed images to see how exposure to transformations through data augmentation can improve model robustness when compared to humans. 
%
%For the following experiments, we consider 14 different image transformations: Shot Noise, Impulse Noise, Gaussian Noise, Glass blur, Gaussian Blur, Defocus Blur, Motion Blur, Brightness and Frost from Imagenet-C~\cite{hendrycks2019robustness}; Blur, Median Blur, Hue Saturation Value and Color Jitter from Albumentations~\cite{albumentation}; and Uniform Noise from Gehiros et. al~\cite{Geirhos2018GeneralisationIH} \red{license?}. To obtain human performance for each transformation, we showed each of 1000 original and 1000 transformed images to five different participants 
%on the Amazon Mechanical Turk platform.\lm{It contradicts the introduction, i.e., 7718 Mechanical turk participants.}\footnote{We paid US$\$0.10$ to classify a batch of 20 images, resulting in estimated hourly wage of US$\$9$, which is above the average US$\$1-6$. Before the experiment, all participants are informed that the data will be used for scientific research. By accepting, completing and submitting a Mturk job, participants consent to data collection. }
%We included qualification tests and sanity checks aimed to filter out participants misunderstanding the task and spammers~\cite{Papadopoulos-et-al-2017}, and only consider results from participants who pass both tests. \lm{This is missing in the experiment subsection.} As a result, we obtained  human predictions for 14,000 ($= 14 \times 1,000$) transformed images and the same number of the original images, for a total of 70,000 ($= 2\time 14 \times 1,000 \times 5$) predictions from 7718 different participants \red{TODO: check this}.
%\red{TODO: I moved human data collected up, probably need another sentence to connect.}
All experiments were conducted on an Intel computer with i7 13700k CPU, Nvidia RTX 4080 GPU with 16GB GRAM, and 32GB of RAM. 
%\purple{We use 8 Imagenet-c transformations:  Gaussian Noise, Shot Noise, Impulse Noise, Defocus Blur, Frosted Glass Blur, Motion Blur, Frost and Contrast, and 2 additional transformations from the Albumentations~\cite{albumentation} library in the same noise and blur class. }
%{\bf MC:  END}

\noindent
\textbf{Verifying Data Transferability.}
%Considering three collections of commonly used image transformations, Albumentations~\cite{albumentation}, included in benchmark Imagenet-c~\cite{hendrycks2019robustness} and Gehiros et. al~\cite{Geirhos2018GeneralisationIH}, the authors identified two classes of similar transformations using the ILSRVR'12 dataset~\cite{ILSVRC2012}: 1) the noise class: Shot Noise, Impulse Noise, Gaussian Noise, Uniform Noise; 2) the blur class: Blur, Median Blur, Glass blur, Gaussian Blur, Defocus Blur; and as comparison, we also included 3) five transformations different from the two similar classes: Motion Blur, Hue Saturation Value, Color Jitter, Brightness and Frost. {\bf MC:  this was an extremely long and unparsable sentence.  please break into several} See supplementary for a demonstration of these transformations.
%\red{TODO: added these non-similar as comparison: Hue Saturation Value and Color Jitter, Motion Blur, brightness and frost. }
%
% \item experiments to support this?
%    \indent\quad Need to verify this assumption (similar transformation $\rightarrow$ similar human performance)
We empirically verify the assumption that human robustness data can be transferred between similar transformations with human robustness data obtained for these transformations. Human robustness data is considered \emph{transferable} between two transformations $T_X^1, T_X^2$ if the differences between the resulting spline curves for human performance ${s^h_a}^1$ and ${s^h_a}^2$, ${s^h_p}^1$ and ${s^h_p}^2$ are not statistically significant, i.e.,
if their $83\%$ confidence intervals overlap~\cite{koenker-94, hu-et-al-22}.
%To verify that human robustness data can be transferred between \emph{similar} transformations, we conducted experiments with Amazon Mechanical Turk for the set of similar transformations identified from imagenet-c: \red{TODO: transformations}. 
%Human performance can be transferred if, when measured, %human robustness is affected similarly by these transformations. 
%After obtaining human data, we plot and smoothed human recognition accuracy against $\Delta_v$ values as shown in Fig.~\ref{fig:similar} for \red{transformation A and B}\footnote{See the rest in supplementary material}. %We then process the result using smoothing splines~\cite{koenker-94} to reduce randomness and remove outliers.  
%The difference between two spline models are considered not statistically significant  
Thus, we obtained the spline curves and their $83\%$ confidence interval for each transformation as shown~\footnote{Due to page limit, we only show ${s^h_a}$; see plots for ${s^h_p}$ in supplementary materials.} in Fig.~\ref{fig:similar}. 
%The spline curves obtained from human performance for the the noise and blur classes of similar transformations are shown in Fig.~\ref{fig:similar}. 
 We can observe that, for all transformations shown, human performance decreases slowly  for small values of visual degrade ($\Delta_v$), but once $\Delta_v$ reaches a turning point, human performance starts decreasing more rapidly. Then, we  observe that spline curves obtained for similar blur and noise transformations have similar shapes, while those for dissimilar transformations start decreasing at different turning points with different slopes. %decrease differently.  
% {\bf MC:  please check that this %is saying the right thing %\blue{updated}}.
 %have different trends which are decreasing in the later half} {\bf MC: ?? \blue{rewritten}}
%different slopes for decreasing 
%
For each pair of similar transformations $T_X^1, T_X^2$ included in our experiment, we verified that the $83\%$ confidence intervals of all similar transformations in the same class overlap. For dissimilar transformations, while the $83\%$ confidence intervals can overlap for certain $\Delta_v$ values, 
they do not overlap when
%\blue{for the most part regarding 
$\Delta_v \geq 0.6$.
%, the intervals do not overlap.}
%the intervals do not overlap for a substantial part at the later half of the curve.
%{\bf MC:  not sure what "substantial part at the later half" means \blue{updated}}
%From Fig.~\ref{fig:similar}, we can see that spline curves for similar transformations have similar trends, and the $83\%$ confidence intervals for similar transformations overlap.
%compared the confidence intervals of the estimated spline curves ${sp^h_a}^1$ and ${sp^h_a}^2$, ${sp^h_p}^1$ and ${sp^h_p}^2$. 
As a result, our experiment showed that, for the similar transformations we identified, the resulting spline curves for human performance are not statistically significant, and thus human data can be transferred between similar transformations.
%for all classes of transformations, we observed that the difference between splines obtained are not statistically significant. %For example, we can see that the spline models obtained for the visually similar transformations Gaussian blur and Median blur in Fig.~\ref{fig:example} are similar as shown in Fig.~\ref{fig:similar}. %Due to page limit, we include the plots and data in supplementary material$^{\ref{gitlink_note}}$. 
%To conclude, experiment results showed that these transformations identified as similar with our method indeed affected human robustness similarly, i.e., resulting in similar curves, thus human data can be transferred between similar transformations. 
Therefore, our method can be used to determine whether new human data is necessary when studying robustness against a new transformation. However, it is reasonable to assume that two transformations can have very different visual effects but still affect human robustness in the same way. Since our method identifies only  transformations with the same visual effects to humans, we are unable to detect such situations.
%this situation cannot be detected with our method. 

%\end{itemize}

%\item how do we verify similarity with IQA?
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/blur_a.png}
         \caption{ \small Blur transformations}
         \label{fig:d}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/noise_a.png}
         \caption{\small Noise transformations}
         \label{fig:d}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/others_a.png}
         \caption{\small Dissimilar transformations}
         \label{fig:d}
     \end{subfigure}
    \caption{\small Comparing human performance spline curves $s^h_a$ for similar and dissimilar transformations. For each curve, the coloured region around the curve is the $83\%$ confidence interval used for comparison of similarity~\cite{koenker-94}.}
    \label{fig:similar}
    %\vspace{-0.25in}
\end{figure}


%- Which models are chosen\\



\noindent
\textbf{Benchmark Robustness against Humans.}
In this experiment, we aim to demonstrate differences between our benchmark and the \SoTA{} benchmark \imagenetc.
%In this experiment, we aim to demonstrate differences between our method and the \SoTA{} benchmark \imagenetc.
Our experiment used all 12 \SoTA{}
%Then, for checking DNN \robustness{} against humans, we used all 12 
DNN models~\cite{pytorch,NoisyMix,GeirhosRMBWB19,HendrycksBMKWDD21,Hendrycks_AugMix,SalmanIEKM20,croce2020robustbench,KrizhevskySH12,tian2022deeper} on the robustbench \imagenetc{} leaderboard~\cite{croce2020robustbench}. These models are optimized against image corruptions in \imagenetc. % Our experiments and model retraining 
We check \robustness{} of these 12 DNN models  against all 9 \imagenetc{} transformations with our generated benchmark validation set and our human-aware metrics \textit{HMRI} and \textit{MRSI}. We then compare results with robust accuracy of the same models on \imagenetc{} images.
%and then compare the results with their corruption robustness evaluated with \imagenetc. 
Since human \robustness{} is measured on 16 entry-level classes,
\textit{HMRI} and \textit{MRSI} are calculated by mapping DNN labels to the same 16 classes for a fair human-DNN comparison.
%For our human-aware metrics \textit{HMRI} and \textit{MRSI}, for a more fair comparison between human and DNNs, we mapped DNN predictions into the 16 entry-level classes human on which \robustness{} is measured. 
 %Mapping to 16 classes would result in higher accuracy and metric values than considering all 1000 classes.  {\bf MC:  not enough info here} 
%Additionally, \imagenetc{} ranks DNNs with accuracy {\bf MC:  what does it mean?} on all transformed images for all transformations, while we consider each transformation separately.  
Results are shown in Tbl.~\ref{tab:eval_results}. We present results for two transformations in this paper; the rest are in the supplementary. %For each transformation, we used test sequences of size $50,000$. 
%\red{TODO: Calculate CO2 Emission}\blue{\bf{[Discussed in supplementary]}}.


First of all, it is essential to test robustness before deploying DNNs into an environment with a wide and continuous range of visual changes. For measuring robust accuracy, \imagenetc{} uses images transformed with five pre-selected parameter values. Our results show that this is not representative of model robustness with respect to the full continuous range of visual change. Consider the transformation Gaussian Noise.  As highlighted in red in Tbl.~\ref{tab:eval_results}, NoisyMix~\cite{NoisyMix} and NoisyMix\_new~\cite{NoisyMix} have
almost the same robust accuracy on \imagenetc{},  but NoisyMix\_new has higher 
%has the highest \imagenetc{} robustness accuracy, but one of the lowest 
$\hat{\robustnesssymbol}^a$; similarly, SIN~\cite{GeirhosRMBWB19} has higher \imagenetc{} robust accuracy but lower $\hat{\robustnesssymbol}^a$ than SIN\_IN\_IN~\cite{GeirhosRMBWB19}.
If we consider transformation Shot Noise, \imagenetc{} ranks
 Do\_50\_2\_Linf~\cite{SalmanIEKM20} second to last,  but its $\hat{\robustnesssymbol}^a$ is around the median. 
%AugMix~\cite{hendrycks2020augmix} and NoisyMix\_new~\cite{NoisyMix} have the same \imagenetc{} robust accuracy but considering a wider range of visual change, AugMix~\cite{hendrycks2020augmix} is more robust with a higher $\hat{\robustnesssymbol}^a$ value.
%AugMix~\cite{hendrycks2020augmix} is ranked in the middle with \imagenetc{} robustness accuracy but it has the highest $\hat{\robustnesssymbol}^a$ among all the DNNs. 
This is because checking robustness on only a portion of the full range of changes, as in \imagenetc, can lead to biased results.  Our benchmark, generated with \method{}, is able to detect such biases. 

Second, in addition to accuracy, our benchmark can also be used to check whether the DNN can preserve its predictions after transformations, i.e., its prediction similarity, which can give us additional information about DNN robustness. As highlighted in green in Tbl.~\ref{tab:eval_results} for the transformation Shot Noise, the model %NoisyMix\_new~\cite{NoisyMix} has a higher $\hat{\robustnesssymbol}^a$ than NoisyMix~\cite{NoisyMix} but a lower $\hat{\robustnesssymbol}^p$; similarity, 
SIN\_IN\_IN~\cite{GeirhosRMBWB19} has a higher $\hat{\robustnesssymbol}^a$ than Standard\_R50~\cite{croce2020robustbench} but a lower $\hat{\robustnesssymbol}^p$. This suggests that even though SIN\_IN\_IN has a better accuracy for transformed images, it labels the same image with different labels before and after transformations. Since ground truth would be hard to obtain during deployment, having low prediction similarity indicates issues with model stability and could raise concerns about when to trust the model prediction. 
%we have an extra measure, prediction similarity,

Third, we also introduced human-aware metrics for comparing model \robustness{} with humans. Since humans are naturally robust to a wide range of changes, using human performance as a baseline can give information about the trustworthiness of DNNs.
Overall,  Tbl.~\ref{tab:eval_results} shows that most \SoTA{} DNNs do not reach human-level \robustness (as measured via our metric \textit{HMRI}), with the exception of Deeper\_DeiT-B~\cite{tian2022deeper} which completely exceeds \robustness{} of an average human regarding prediction similarity (see Fig.~\ref{fig:gauss_noise_s1}). Additionally, our metric \textit{MRSI} tells us that  whether DNNs can outperform humans
with respect to certain levels of visual changes. As highlighted in blue in Tbl.~\ref{tab:eval_results}, for $\hat{\robustnesssymbol}^p$ of Shot Noise, H\_Many~\cite{HendrycksBMKWDD21} is more robust than AugMix~\cite{Hendrycks_AugMix} compared to humans (i.e., has higher \textit{HMRI} values).  Yet  \textit{MRSI} values indicate that AugMix outperforms humans for certain levels of visual change, while H\_Many does less so. 
By visualizing the spline curves obtained for these two models in Fig.~\ref{fig:shot_noise_s1}, we  see that this is because AugMix has a better prediction similarity with a higher confidence than H\_Many for lower levels of visual change, but a lower prediction similarity for higher levels of visual change starting approximately from $\Delta_v = 0.5$. Thus, AugMix is a better fit for environments with more low-level visual changes. 
%Comparison with humans can give information about trustworthiness of the DNNs.
%; while SIN has lower accuracy throughout the entire visual change range and as a result has higher accuracy than humans for high levels of visual change. 
%Similarly regarding $\robustnesssymbol_p$ and Defocus Blur, Deeper\_DeiT-B has higher \textit{HMRI} than Deeper\_DeiT-T, but Deeper\_DeiT-T outperforms human more when visual change is close to 1, as shown in Fig.~\ref{fig:defocus_blur_s1} and Fig.~\ref{fig:defocus_blur_s2}.

%By visualizing the spline curves used to calculate \textit{HMRI} and \textit{MRSI}, as shown in Fig.~\ref{fig:spline_results}, we can identify the specific range of visual change for which DNNs can outperform humans. %Such information can be useful 
%we can see model performance vs humans and when a model outperforms humans, use plot to demonstrate (blue)

Additionally, we  see that Gaussian Noise and Shot Noise are similar transformations for humans but not for DNNs. For example, for Do\_50\_2\_Linf~\cite{SalmanIEKM20}, it is ranked second to last for $\robustnesssymbol_a$ for Gaussian Noise but in the middle for Shot Noise.
To conclude, compared to \imagenetc, our benchmark checks \robustness{} on the full range of visual changes, gives information about model stability when ground truth is not easily attainable, and compares DNN \robustness{} to humans. 

 
%Since human \robustness{} is measured on 16 entry-level labels, for a more fair comparison between human and DNNs, our human-aware metrics $HMRI$ and $MRSI$ are measured by mapping DNN predictions into the 16 entry-level classes. Unlike Imagenet-C, we present results for each transformation separately in Tbl.~\ref{tab:eval_results}. 



%\red{TODO: $mCE$ is correlated with accuracy, we provide comparison on supplementary}
%Standard accuracy is produced with the validation set of ImageNet 2022 ($acc=P(f(x_i) == f^*(x_i))$). Robust accuracy is produced by evaluating against the entire ImageNet C dataset with all 5 levels of transformations. Visual-change robustness regarding accuracy $P^a_{h-m}$, and \robustness regarding prediction similarity $P^p_{h-m}$ is produced by evaluating the accuracy against image benchmark generated using the method mentioned in section \ref{section:benchmark-generation} and metrics defined in section \ref{sec:eval-metrics}.
%ImageNet has 1000 classes and it is impossible to conduct human experiments on 1000 classes. Instead, we use the 16-class-ImageNet~\cite{Geirhos2018GeneralisationIH}, which consists of 16 general classes, for human to classify. The data we used comes from ImageNet 2012. Predictions of ML models are mapped to the 16 classes before accuracy is calculated. Each transformation and metric has a unique value in the evaluation. The evaluation does not aggregate over transformations. The results can be found in Table \ref{tab:eval_results}. 


%\begin{itemize}
    %\item Their tests do not cover visual change (not representative), our coverage VS their coverage
%    \item Their checking does not show comparison with humans (models good on their benchmark might not be good on ours) -> simply comparing accuracy is not enough, comparing with humans is another layer of contribution
%    \item What can we learn about the models using our benchmarks: some models are accuracy but cannot preserve their labels, some models are better at certain range of visual change etc. 
%\end{itemize}

%- Detailed experiments result \red{TODO: imagenet c values}\\
%- Compare with benchmarks\\
%\indent\quad - Evaluate using old and new metric\\

\noindent
\textbf{Training with Data Augmentation.} Training models optimized for \imagenetc{} with transformed images generated by us on the entire visual change range can result in better robustness compared to humans, i.e.,  with higher \textit{HMRI} and \textit{MRSI} values. Due to the page limit, we include results and details of training in supplementary material.
%\begin{itemize}
%    \item Show that our benchmark images can be used to improve robustness
%    \item \red{check Gehiros' work on retraining, add table...}
%\end{itemize}

%Beyond evaluating existing models on robustbench~\cite{croce2020robustbench}, retraining and evaluation are also conducted on these models using our generated images. \SoTA{} models included in Tbl.~\ref{tab:eval_results} are optimized for ImageNet-C, which only included images transformed a few fixed transformation levels. 
%Training models optimized for ImageNet-C with transformed images we generated on the entire visual change range resulted in better robustness compared to humans, i,e, higher \textit{HMRI} and \textit{MRSI} values \red{TODO: improved by how much (image?)}.
%Training models on a few fixed transformation levels could potentially introduce bias in robustness evaluation. Our generated training data is on the entire visual change range and we expect to see better results when models are evaluated on our generated benchmark comparing to the original models (optimized for ImageNet-C).\\
%The evaluation in this section is for comparing models before and after training on our generated benchmark dataset. Therefore, we do not need to use the 16 general classes designed for humans. Instead, robustness metrics were directly computed based on the 1000 ImageNet classes.
%Due to page limit, we include details of this experiment and results in supplementary materials.

%Evaluation results can be found in table \ref{tab:eval_results}. \blue{TODO: Does robustness metrics improve with the new training data? Describe the results.} 

% checkout 2.4 of  \url{https://arxiv.org/pdf/1808.08750.pdf}


\input{sections/evaluation_table}


\begin{comment}

\subsection{\blue{Table Format Instructions:}}
All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}


\end{comment}


% \begin{tabular}{ |l|l|l| }
% \hline
% \multicolumn{3}{ |c| }{Team sheet} \\
% \hline
% Goalkeeper & GK & Paul Robinson \\ \hline
% \multirow{4}{*}{Defenders} & LB & Lucas Radebe \\
%  & DC & Michael Duburry \\
%  & DC & Dominic Matteo \\
%  & RB & Didier Domi \\ \hline
% \multirow{3}{*}{Midfielders} & MC & David Batty \\
%  & MC & Eirik Bakke \\
%  & MC & Jody Morris \\ \hline
% Forward & FW & Jamie McMaster \\ \hline
% \multirow{2}{*}{Strikers} & ST & Alan Smith \\
%  & ST & Mark Viduka \\
% \hline
% \end{tabular}


%For the set of transformations for image corruption included in benchmark Imagenet-c, we identified 2 classes of similar transformations: the noise class, Gaussian Noise, Shot Noise, Impulse Noise; and the blur class Defocus Blur, Frosted Glass Blur, Motion Blur. These two classes are identified through experiments with the ILSRVR'12 dataset using $N=10$ with 2 of the authors of the paper. The experiment took on average 5 minutes per participant. Notice that the entire experiment is fully randomized to minimize bias. 



==> sections/evaluation_table.tex <==
\newcolumntype{g}{>{\columncolor{gray!10}}c}


\begin{table*}[t]
    \centering

\noindent\scalebox{0.57}{
    \begin{tabular}{ >{\columncolor{gray!10}}c c c c c c c c >{\columncolor{gray!25}}c c c c c c c c  }
    \hline
         & & \multicolumn{6}{c}{Our benchmark}& & & \multicolumn{6}{c}{Our benchmark}\\
        \cline{3-8} \cline{11-16}
           &  & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Prediction similarity}&  &  & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Prediction similarity}\\
        \cline{3-8} \cline{11-16}
        \multirow{-3}{*}{DNN} &  \multirow{-3}{*}{\shortstack{SoTA\\ robust \\acc}} & $\hat{\robustnesssymbol}_a$& HMRI & MRSI & $\hat{\robustnesssymbol}_p$& HMRI & MRSI& \multirow{-3}{*}{DNN} & \multirow{-3}{*}{\shortstack{SoTA\\ robust\\ acc}} & $\hat{\robustnesssymbol}_a$& HMRI & MRSI & $\hat{\robustnesssymbol}_p$& HMRI & MRSI\\
        
        \hline
           \multicolumn{8}{c}{\cellcolor{gray!15}\shortstack{\textbf{Gaussian Noise}}} & \multicolumn{8}{c}{\cellcolor{gray!30}\shortstack{\textbf{Shot Noise}}}\\
        \hline
        \cellcolor{blue!15} Deeper\_DeiT-B~\cite{tian2022deeper} & 0.763 & 0.831 &0.949 & 0.055 & 0.927& \cellcolor{blue!15}1.000 & \cellcolor{blue!15}0.102
        & Deeper\_DeiT-B  & 0.767 & 0.799 & 0.914 & 0.036 & 0.871 & 0.943 & 0.061\\
        \hline
        Deeper\_DeiT-S~\cite{tian2022deeper}  & 0.724 & 0.787 & 0.925 & 0.027 &0.887 & 0.996 & 0.065
        & Deeper\_DeiT-S & 0.727 & 0.767 & 0.876 & 0.038 & 0.840 & 0.920 & 0.050\\
        \hline  
        H\_Many~\cite{HendrycksBMKWDD21}  & 0.566 & 0.666 & 0.804 & 0.000 & 0.769 & 0.901 & 0.025
        & \cellcolor{blue!15} H\_Many &0.548 & 0.712 & 0.811 & 0.040 & 0.754 & \cellcolor{blue!15}0.845 & \cellcolor{blue!15}0.029\\ 
        \hline
        \cellcolor{red!15} NoisyMix~\cite{NoisyMix} & \cellcolor{red!15} 0.531 & \cellcolor{red!15} 0.639 & 0.772 & 0.000 & 0.750 & 0.864 & 0.041
        &  NoisyMix & 0.525 &  0.685 & 0.779 & 0.042 & 0.732 & 0.818 & 0.030\\
        \hline
       \cellcolor{red!15} NoisyMix\_new~\cite{NoisyMix} & \cellcolor{red!15} 0.530 & \cellcolor{red!15} 0.668 & 0.807 & 0.000 & 0.782 & 0.895 & 0.047
       &  NoisyMix\_new  & 0.519 & 0.691 & 0.787 & 0.042 & 0.763 & 0.838 & 0.048\\
        \hline
        SIN\_IN~\cite{GeirhosRMBWB19} & 0.413 & 0.605 & 0.730 & 0.000 & 0.701 & 0.831 & 0.013
        & \cellcolor{blue!15}AugMix & 0.411 & 0.655 & 0.743 & 0.044 & 0.719 & \cellcolor{blue!15}0.792 & \cellcolor{blue!15}0.045 \\
        \hline
        AugMix~\cite{Hendrycks_AugMix}  & 0.406 & 0.608 & 0.735 & 0.000 & 0.700 & 0.823 & 0.021
        & SIN\_IN  & 0.403 & 0.547 & 0.650 & 0.000 & 0.600 & 0.692 & 0.000\\
        \hline
        Resnet50~\cite{pytorch} & 0.379 & 0.591 & 0.713 & 0.000 & 0.674 & 0.797 & 0.015 
        &  Resnet50  & 0.354& 0.533 & 0.633 & 0.000 & 0.565 & 0.652 & 0.000\\
        \hline
        \cellcolor{red!15} SIN~\cite{GeirhosRMBWB19} & \cellcolor{red!15} 0.369 & \cellcolor{red!15} 0.515 & 0.622 & 0.000 & 0.660 & 0.787 & 0.005
        & \cellcolor{red!15} SIN & \cellcolor{red!15} 0.344 & \cellcolor{red!15} 0.472 & 0.560 & 0.000 & 0.555 & 0.640 & 0.000\\
        \hline
        \cellcolor{red!15} SIN\_IN\_IN~\cite{GeirhosRMBWB19} & \cellcolor{red!15}0.327 & \cellcolor{red!15}0.585 & 0.707 & 0.000 & 0.668 & 0.791 & 0.013
        & \cellcolor{green!15}SIN\_IN\_IN& 0.312 &\cellcolor{green!15} 0.523 & 0.621 & 0.000 & \cellcolor{green!15}0.649 & 0.723 & 0.034\\
        \hline
        Standard\_R50~\cite{croce2020robustbench} & 0.293 & 0.567 & 0.685 & 0.000 & 0.656 & 0.774 & 0.017
        &\cellcolor{green!15} Standard\_R50 & 0.270 & \cellcolor{green!15}0.505 & 0.599 & 0.000 & \cellcolor{green!15}0.654 & 0.723 & 0.041\\
        \hline
        Do\_50\_2\_Linf~\cite{SalmanIEKM20} & 0.260 & 0.490 & 0.592 & 0.000 & 0.635 & 0.733 & 0.039
        & \cellcolor{red!15} Do\_50\_2\_Linf  &\cellcolor{red!15} 0.245 & \cellcolor{red!15} 0.560 & 0.630& 0.051 & 0.603 & 0.671 & 0.036\\
        \hline
        AlexNet~\cite{KrizhevskySH12} & 0.114 & 0.374 & 0.452 & 0.000 & 0.538 & 0.639 & 0.009
        & AlexNet & 0.106 &0.351 &0.416 & 0.000 & 0.536 & 0.592 & 0.042\\
        \hline
        
        %\hline
         %\multicolumn{8}{c}{\cellcolor{gray!15}\shortstack{\textbf{Brightness}}} & \multicolumn{8}{c}{\cellcolor{gray!30}\shortstack{\textbf{Frost}}}\\
        %\hline
        %\cellcolor{blue!15} Deeper\_DeiT-B & 0.791 & 0.789 &\cellcolor{blue!15} 0.900 & \cellcolor{blue!15}0.000 & 0.876& \cellcolor{blue!15}0.970 & \cellcolor{blue!15}0.055
        %& Deeper\_DeiT-B  & 0.709 & 0.667 & 0.774 & 0.056 & 0.717 & 0.823 & 0.062\\
        %\hline
        %Deeper\_DeiT-S  & 0.763 & 0.760 & 0.900 & 0.000 &0.854 & 0.949 & 0.051
        %& Deeper\_DeiT-S & 0.667 & 0.608 & 0.711 & 0.049 & 0.672 & 0.776 & 0.057\\
        %\hline  
        %Resnet50 & 0.721 & 0.707 & 0.837 & 0.000 & 0.800 & 0.900 & 0.040
        %& NoisyMix\_new  & 0.527 & 0.503 & 0.595 & 0.037 & 0.563 & 0.659 & 0.043\\
        %\hline
        %NoisyMix & 0.711 & 0.701 & 0.830 & 0.000 & 0.800 & 0.897 & 0.042
        %& NoisyMix & 0.526 & 0.503 & 0.596 & 0.037 & 0.565 & 0.661& 0.043\\
        %\hline
       %\cellcolor{blue!15}  H\_Many  & 0.711 & 0.708 & 0.838 & 0.000 & 0.802 & 0.908 & 0.033
       %& H\_Many &0.503 & 0.471 & 0.559 & 0.033 & 0.517 & 0.609 & 0.038\\ 
        %\hline
        %\cellcolor{blue!15} NoisyMix\_new & 0.710 & 0.702 & 0.682 & 0.000 & 0.801 & 0.901 & 0.041  
        %&  Resnet50  & 0.467 & 0.453 & 0.540 & 0.031 & 0.509 & 0.600 & 0.036\\
        %\hline
        %AugMix  & 0.695 & 0.674 & 0.798 & 0.000 & 0.763 & 0.863 & 0.035
        %& AugMix& 0.438 & 0.439 & 0.524 & 0.029& 0.482 & 0.570 & 0.034 \\
        %\hline
        %SIN\_IN\_IN & 0.686 & 0.672 & 0.795 & 0.000 & 0.757 & 0.862 & 0.028
        %& SIN\_IN  & 0.416 &0.417 & 0.498 & 0.027 & 0.461 & 0.547 & 0.032\\
        %\hline
        %Standard\_R50 & 0.680 & 0.654 & 0.775 & 0.000 & 0.746 & 0.849 & 0.029
        %& SIN\_IN\_IN& 0.403 & 0.418 & 0.501 & 0.025 & 0.455 & 0.541 & 0.029\\
        %\hline
        %SIN\_IN & 0.674 & 0.676 & 0.801 & 0.000 & 0.773 & 0.880 & 0.028
        %& SIN &0.385 & 0.386 & 0.463 & 0.023 & 0.459 & 0.544 & 0.031\\
        %\hline
        %Do\_50\_2\_Linf & 0.590 & 0.554 & 0.656 & 0.000 & 0.663 & 0.760 & 0.021
        %& Standard\_R50 & 0.381 & 0.381 & 0.458 & 0.023 & 0.420 & 0.501 & 0.025\\
        %\hline
        %\cellcolor{green!15}  SIN & 0.554 & \cellcolor{green!15} 0.576 & 0.682 & 0.000 & \cellcolor{green!15} 0.729 & 0.842 & 0.013
        %& Do\_50\_2\_Linf  &0.351 & 0.303 & 0.367 & 0.013 & 0.356 & 0.428 & 0.019\\
        %\hline
        %AlexNet & 0.435 & 0.414 & 0.490 & 0.000 & 0.550 & 0.636 & 0.012
        %& AlexNet & 0.173 &0.191 &0.234 & 0.004 & 0.245 & 0.297 & 0.009\\
        %\hline
        
        
        \multicolumn{12}{l}{Note: all numbers are rounded.}
    \end{tabular}
}
    \caption{Measuring \robustness{} of leaderboard~\cite{croce2020robustbench} DNNs for the \SoTA{} benchmark  \imagenetc~\cite{hendrycks2019robustness}. }
    \label{tab:eval_results}
    \vspace{-0.1in}
\end{table*}


\begin{comment}

\begin{figure}[ht]
\centering
\scalebox{0.9}{
    \begin{tabular}{c | c c }
    
    $s_p^m$ for Gaussian Noise &  \multicolumn{2}{c}{$s_p^m$ for Shot Noise}\\
        \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/model-vs-human-plots/pred-sim_Tian2022Deeper_DeiT-B.png}
         \caption{ \small Deeper\_DeiT-B~\cite{tian2022deeper}}
         \label{fig:glass_blur_s1}
     \end{subfigure} &
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/model-vs-human-plots/pred-sim_Hendrycks2020AugMix.png}
         \caption{ \small AugMix~\cite{Hendrycks_AugMix}}
         \label{fig:defocus_blur_s1}
     \end{subfigure} &
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{resources/model-vs-human-plots/pred-sim_Hendrycks2020Many.png}
         \caption{\small  H\_Many~\cite{HendrycksBMKWDD21}}
         \label{fig:defocus_blur_s2}
     \end{subfigure}
    \end{tabular}
}
     
\caption{\small Comparison of spline curves of DNNs \robustness{} with Humans. 
The coloured region around each curve is the $95\%$ confidence interval.
%Model evaluation comparing with human performance. 
\red{TODO: update this figure, merge plots for the same transformation + legend}}
\label{fig:model-vs-human-plots}
\end{figure}


\end{comment}

\begin{figure}[t]
	\centering
    \begin{subfigure}{.35\textwidth}
		\includegraphics[width=\textwidth]{resources/model-vs-human-plots/gaussian_noise_pred-sim_Tian2022Deeper_DeiT-B.png}
		\caption{$s_p^m$ for Gaussian Noise}
		\label{fig:gauss_noise_s1}
	\end{subfigure}
	\begin{subfigure}{.35\textwidth}
		\includegraphics[width=\textwidth]{resources/model-vs-human-plots/shot_noise_pred-sim_compare_Hendrycks2020AugMix_vs_Hendrycks2020Many.png}
		\caption{$s_p^m$ for Shot Noise}
		\label{fig:shot_noise_s1}
	\end{subfigure}
	\caption{\small Comparison of spline curves of DNNs \robustness{} with Humans. 
The coloured region around each curve is the $95\%$ confidence interval.
%Model evaluation comparing with human performance. 
}
\vspace{-0.15in}
\end{figure}








\begin{comment}

\begin{table*}[t]
    \centering

\noindent\scalebox{0.58}{
    \begin{tabular}{ >{\columncolor{gray!15}}c c c c c g g g g >{\columncolor{gray!30}}c c c c c g g g g }
    \hline
        \multicolumn{9}{c}{\cellcolor{gray!15}\shortstack{\textbf{Uniform Noise}}} &\multicolumn{9}{c}{\cellcolor{gray!30}\shortstack{\textbf{Medium Blur}}} \\
        \hline
        & \multicolumn{4}{c}{Original model} & \multicolumn{4}{g}{Retrained model} & & \multicolumn{4}{c}{Original model} & \multicolumn{4}{g}{Retrained model}\\
        \cline{2-9}\cline{11-18}
         &   \multicolumn{2}{c}{$\robustnesssymbol_a$} & \multicolumn{2}{c}{$\robustnesssymbol_p$}&   \multicolumn{2}{g}{$\robustnesssymbol_a$} & \multicolumn{2}{g}{$\robustnesssymbol_p$} &
         &   \multicolumn{2}{c}{$\robustnesssymbol_a$} & \multicolumn{2}{c}{$\robustnesssymbol_p$}&   \multicolumn{2}{g}{$\robustnesssymbol_a$} & \multicolumn{2}{g}{$\robustnesssymbol_p$}\\
        \cline{2-9}\cline{11-18}
        \multirow{-4}{*}{DNN} &  HMRI & MRSI & HMRI & MRSI&  HMRI & MRSI & HMRI & MRSI & \multirow{-4}{*}{DNN} &  HMRI & MRSI & HMRI & MRSI&  HMRI & MRSI & HMRI & MRSI\\
        
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
        Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2 & Standard R50 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5 & 0.75 & 0.2\\
        \hline
        model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 & model 2 & 0.75 & 0.2 & 0.5 & 0.5 & 0.6 & 0.5& 0.75 & 0.2 \\
        \hline
    \end{tabular}
}
    \caption{Results for retraining \red{placeholder, another way to display this?}.}
    \label{tab:retraining_results}
\end{table*}

\end{comment}


\begin{comment}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/retraining.png}
         \caption{ \small Uniform Noise}
         \label{fig:d}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/retraining.png}
         \caption{\small Medium Blur}
         \label{fig:d}
     \end{subfigure}
     
    \caption{\small Our human-aware metrics HMRI and MRSI for DNNs shown in Tbl.~\ref{tab:eval_results} finetuned with our benchmark data. \red{placeholder, can also split HMRI and MRSI, to include more transformations in a figure, put tables in supplementary material}}
    \label{fig:retraining_results}
\end{figure}

\end{comment}


==> sections/experiments.tex <==
\section{Measuring Human Robustness}
\label{sec:experiments}

%\red{both human and ML test images should be separated by v value, according to the definition. Then we plot it like this....}

Step~\RN{2} of our approach is to obtain human robustness performance data (Fig.~\ref{fig:intro-paper-design-flowchart}) for robustness comparison with DNNs. Human performance is currently measured through experiments with human participants. The objective of such experiments is to measure how human recognition performance is affected as changes in images increase as the result of applying transformations. In this section, we introduce the experiment setup to measure human robustness; and our method for identifying similar transformations for transferring data.  The method for identifying similar transformations is implemented as part of {\method} to allow  users to check whether new human data is needed for a new transformation. 
% and describe the data we collected. 
 %\footnote{Implementation of the experiment and data can be found in supplementary materials.}

\noindent
\textbf{Experiment Setup.}
The experiment is designed following Hu et al.~\cite{hu-et-al-22} and Geirhos et al.~\cite{Geirhos2018GeneralisationIH}. 
The experiment procedure is a \emph{forced-choice image categorization task}: humans are presented with one image at a time, for 200 ms, and asked to choose one of the given labels (e.g., car or bird)~\cite{Geirhos2018GeneralisationIH}. The ILSRVR'12 dataset~\cite{ILSVRC2012} has 1,000 fine-grained classes; however, humans, when asked to label, are only able to categorize objects into entry-level classes (e.g., a dog rather than a German shepherd)~\cite{Geirhos2018GeneralisationIH}. Therefore, we provide humans with the  16 entry-level class labels mapped by Geirhos et al.~\cite{Geirhos2018GeneralisationIH}: airplane, bicycle, boat, car, chair, dog, keyboard, oven, bear, bird, bottle, cat, clock, elephant, knife, truck. The time to classify each image is set to ensure fairness in the comparison between humans and machines~\cite{Firestone26562}. Between images, we show a noise mask to minimize feedback influence in the brain~\cite{Geirhos2018GeneralisationIH}. %\lm{The qualification tests are not mentionned.} \blue{see below}

The experiment takes as inputs 1) a transformation $T_X$; 2) a dataset of original images $\{x\}$, $x\sim P_X$, with their ground-truth labels $\{f^*(x)\}$; 3) a parameter domain $C$ for each transformation parameter. Then, we obtain a validation set of $\{(x, x')\}, x'=T(x,c), c\sim \textit{Uniform}(C)$. Human predictions are collected for both original ($x$) and transformed images ($x'$), and a given subject is never shown more than one version of $x_i$, whether original or transformed. 
Then, for measuring $\robustnesssymbol_a$ [resp. $\robustnesssymbol_p$], human performance data is processed to obtain the spline curve $s^h_a$ [resp. $s^h_p$] representing the relationship between human accuracy [resp. prediction similarity] and $\Delta_v$ values.  The curves $s^h_a$ and $s^h_p$ are used for the comparison of DNN \robustness{} with humans (in Step~\RN{3} of Fig.~\ref{fig:intro-paper-design-flowchart}), i.e., $s^h_a$ and $s^h_p$ are compared with the curves of DNNs $s^m_a$ and $s^m_p$, respectively.
%and are encouraged to sign up to receive updates 

%\red{TODO: what is the human data included in our benchmark for comparison and how are they obtained (moved from evaluation).}

\noindent
\textbf{Human Data Collected.} %\blue{\textbf{[NOTE: this part is moved from evaluation up here]}}
We measured human performance for all 14 transformations included in the validation set of our benchmark.
To obtain human performance for each transformation, we showed each of the $1{,}000$ original and $1{,}000$ transformed images to five different participants
on the Amazon Mechanical Turk platform. One job on Mturk includes classifying a batch of 20 images, which takes approximately $40\,s$ to complete. We paid US$\$0.10$ for one job, resulting in estimated hourly wage of US$\$9$, which is above the average US$\$1$-$6$. Thus, for each transformation, obtaining human classification  takes at least $5.55$ hours ($2{,}000 * 5 / 20 * 40\,s = 20{,}000\,s =5.55$ hr).
Before the experiment, all participants were informed that the data would be used for scientific research. By accepting, completing and submitting a Mturk job, participants consented to data collection. 
We included qualification tests and sanity checks aimed to filter out participants misunderstanding the task and spammers~\cite{Papadopoulos-et-al-2017}, and only considered results from participants who passed both tests. As a result, we had $7{,}718$ participants and  obtained approximately (1) $70{,}000$ human predictions on ($= 14 \times 1{,}000 \times 5$) transformed images; and (2) $50{,}000$ on original images as these can be repeated in experiments for different transformations. Then we estimated $s^h_a$ and $s^h_p$ for all 14 transformations.
%As a result, we obtained human predictions for 14,000 ($= 14 \times 1,000$) transformed images and the same number of the original images, for a total of 70,000 ($= 2\time 14 \times 1,000 \times 5$) predictions from 7718 different participants \red{TODO: check this}. 
%\lm{It contradicts the introduction, i.e., 7718 Mechanical turk participants.} \blue{[updated]}
%\noindent
%\textbf{Identify Classes of Similar Transformations.}
%\begin{itemize}
%    \item How do we define similarity
%Different image transformations can impact human perception differently, e.g., changing colour, brightness, thus human robustness is typically measured per transformation~\cite{hu-et-al-22}. Conducting experiments to obtain human robustness data for every new transformation is expensive and time-consuming. However, for transformations that impact human perceptions \emph{similarly}, human robustness data can be transferred between the transformations.

\noindent
\textbf{Transferring Human Robustness Data.}
Different transformations change different aspects of the images, e.g., image colour, contrast and the amount of additive visual noise, and thus affect human perception differently~\cite{Geirhos2018GeneralisationIH}. Also, multiple different transformations can be implemented for the same visual effect, such as Gaussian blur and Glass blur for image blurring as shown in Fig.~\ref{fig:example}. Although the difference between Gaussian blur and Median blur can be picked up by complex DNN models, an average human %without high computational power 
would struggle to distinguish between the two. Therefore, for a specific visual effect, we say that there exists a class of transformations implementing it if an average human is unable to tell them apart. We call transformations in the same class \emph{similar}. We postulate that since similar transformations, by definition, affect human perception similarly, they would affect human robustness similarly as well, and thus
%Similar transformations affect human perception similarly, therefore should affect human robustness similarly. As a result, 
human data for one transformation can be transferred to other similar transformations in the same class. 

%    \item How to check similarity with humans?
%    \item Distribution of image sampling
To identify whether two transformations $T^1_X$ and $T_X^2$ are similar enough to reuse human data, we need to determine whether the difference between them is distinguishable to a human. This can be done through the following  set of relatively inexpensive experiments where the participants are shown transformed images and asked whether the presented images are transformed with the same transformation. Participants are expected to have normal eyesight and a basic knowledge of image transformations. 
%For each pair of transformations, reviewing images 
%this experiment requires each participant to review less than 50 pairs of images, which takes less than a minute. For each transformation, 
%Similar to the full experiment, each set of experiment should be repeated with at least give different participants. 
%One experiment for identifying and reusing human data for a similar transformation requires 40 pairs of images, taking approximately $40\,s$ and can be done by a single participant. 
% \kc{Add quantification for both these and the experiments we try to avoid to make the savings explicit} \blue{added}

%To identify whether two transformations are similar, two things need to be checked: whether humans are able to tell the difference between two transformations, whether the degree of changes is distributed similarly. 
%This can be identified with a small set of experiments with a human. 
%for each transformation $T_X\in \mathbb{T}$ with the parameter domains $C$ and distribution $P_C$, 
%$N$ original images $x_i \sim P_X$ are randomly selected and 
First, $N$ transformed images $x'$ are generated by transforming $x\sim P_X$ with $c \sim \textit{Uniform}(C)$, that is, $x' = T_X(x, c)$ for both $T_X^1$ and $T_X^2$. $N$ should be large enough to obtain results with statistical significance. In our experiments, we used $N=20$. For efficiency, all changes in $x'$ should be clearly visible to the participants, thus, in this paper we use $\Delta_v(x, x') >= 0.8$ for all $x'$. This number can be adjusted as needed to make changes visible in the target dataset.
%Then, we check the similarity of every $T_X^1, T_X^2 \in \mathbb{T} \times \mathbb{T}$ in the process of the experiment. 
The participants are shown two images side by side: $x'^1$ transformed with $T_X^1$ and $x'^2$ transformed with $T_X^2$.  They are asked whether the pair of images presented are transformed with the same transformation, i.e., whether they think that $T_X^1 = T_X^2$. The experiment includes the same number of image pairs where $T_X^1 = T_X^2$ and $T_X^1 \neq T_X^2$. If $T_X^1$ and $T_X^2$ are similar, the participants would only be able to distinguish them with close to random accuracy, which is $0.5$. %\blue{Similar to the full set of experiment measuring human performance, each pair of images should be shown to five different participants.}
%{\bf MC:  why this number? \purple{because the experiment is distinguishing two transformations at a time, if two transformations are similar, human cannot tell them apart}
%}
For each pair of $T_X^1$ and $T_X^2$, we use a binomial test with $p=0.5$ to test whether the null hypothesis `human cannot correctly distinguish between $T_X^1$ and $T_X^2$, i.e., accuracy$=0.5$' holds for the human opinion we observed in the experiments. The null hypothesis is accepted if $p$-value is $\geq 0.95$, meaning that the participants cannot tell the two transformations apart, and thus they are similar. This is an indication that human robustness data can be reused for these two similar transformations. 
A transformation belongs to a class of similar transformations if it is similar to every transformation in the class.  

Our experiments showed that for each pair of transformations, results with statistical significance can be reached in less than a minute. Compared to the full set of experiment with $2{,}000$ images and five different participants for each experiment, identifying similar transformations significantly decreased the experiment time from approximately $5.55$ hours to $5$ minutes.

\noindent
\textbf{Similar Transformations Identified.}
%\red{TODO: which transformations out of what we included are similar and how they were detected}
We identified two classes of similar transformations:
 (1) the noise class with transformations: Shot Noise, Impulse Noise, Gaussian Noise and Uniform Noise; and (2) the blur class with transformations: Blur, Median Blur, Gaussian Blur (Fig.~\ref{fig:b}), Glass blur (Fig.~\ref{fig:c}), Defocus Blur. The remainder of the 14 transformations we considered are dissimilar: Motion Blur (Fig.~\ref{fig:d}), Hue Saturation Value, Color Jitter, Brightness (Fig.~\ref{fig:e}) and Frost. See Fig.\ref{fig:transf_example} for the full demonstration.
%Considering three collections of commonly used image transformations, Albumentations~\cite{albumentation}, included in benchmark Imagenet-c~\cite{hendrycks2019robustness} and Gehiros et. al~\cite{Geirhos2018GeneralisationIH}, the authors identified two classes of similar transformations using the ILSRVR'12 dataset~\cite{ILSVRC2012}: 1) the noise class: Shot Noise, Impulse Noise, Gaussian Noise, Uniform Noise; 2) the blur class: Blur, Median Blur, Glass blur, Gaussian Blur, Defocus Blur; and as comparison, we also included 3) five transformations different from the two similar classes: Motion Blur, Hue Saturation Value, Color Jitter, Brightness and Frost. {\bf MC:  this was an extremely long and unparsable sentence.  please break into several}


%We measured human performance on 14 image transformations~\cite{hendrycks2019robustness,albumentation,Geirhos2018GeneralisationIH}: ISO Noise, Shot Noise, Impulse Noise, Gaussian Noise, Uniform Noise, Blur, Median Blur, Zoom Blur, Glass blur, Gaussian Blur, Defocus Blur, Motion Blur, Brightness and Frost. For each transformation, we included 1000 original and 1000 transformed images, and each image is shown in 5 different participants on the Amazon Mechanical Turk platform. We included qualification tests and sanity checks aimed to filter out participants misunderstanding the task and spammers~\cite{Papadopoulos-et-al-2017}, and only consider results from participants who pass both tests. As a result, collect human predictions for 14,000 ($= 14 \times 1,000$) transformed images and the same number of the original images, for a total of 70,000 ($= 2\time 14 \times 1,000 \times 5$) predictions from \red{number} different participants.







%Then, a sample of original-transformed image pairs $\{(x_i,x_{i,j}’)\}$, $(x_i,x_{i,j}’)\sim P_{T_X}$ are generated by randomly sampling $x_i$ from $\{x_i\}$ and $c_j\sim P_C$, and transforming $x_{i,j}’=T_X(x_i,c_j)$. We ensure that the full range of achievable $\Delta_v$ values is covered when sampling from $P_C$.

%However, in contrast to the work by Geirhos et al., we ensure that the full range of achievable $\Delta_v$ values is covered when sampling from $P_C$, and we also collect human predictions for the original images, so that we can estimate prediction preservation. A given subject is never shown more than one version of $x_i$, whether original or transformed. Note that human predictions for originals are different from their ground truth labels: labelers take as long as needed per image to classify it, but our subjects have only 200 ms to see each image.
%The human data is specific to a task, an image distribution, and a class of transformations, and thus has to be collected for the combination of the three. 

%Note that human predictions for originals are different from their ground truth labels: labelers take as long as needed per image to classify it, but our subjects have only 200 ms to see each image.
%The human data is specific to a task, an image distribution, and a class of transformations, and thus has to be collected for the combination of the three. 

%\red{TO ADD: correspond back to robustness definition, each point on the resulting curve is $P_{x, x'\sim P(x,x'|v)} (f(x') = f*(x))$, the expectation of all of that within $v\in [0,1]$ is done through integral under the curve. (why are we plotting this way)}

%\noindent
%\textbf{Data Collection and Processing.} We obtained human robustness data for 8 transformations from the benchmark Imagenet-C~\cite{hendrycks2019robustness}: Gaussian Noise, Shot Noise, Impulse Noise, Defocus Blur, Frosted Glass Blur, Motion Blur, Frost and Contrast. For each transformation, we sampled 1000 transformed images $x_{i,j}’$ from the ILSRVR'12 dataset, and have each image labeled by five humans. To achieve this, we divide the 2,000 (transformed and original images) $\times$ 8 ($\#$considered) transformations into batches of 20 images. Each batch is shown five times to different participants using the platform Amazon Mechanical Turk. We include qualification tests and sanity checks aimed to filter out participants  misunderstanding the task and spammers~\cite{Papadopoulos-et-al-2017}, and only consider results from participants who pass both tests.
%\red{TODO: update with real experiment}
%As a result, we used $\{x_i\}$ with 13,000 car images and same number of non-car images, and collect human predictions for 40,000 ($= 5 \times 8 \times 1,000$) transformed images and the same number of the original images, for a total of 80,000 predictions. \red{TODO: update with new experiment} 


%Following~\cite{hu-et-al-22}, the human predictions collected are further processed to obtain functions to represent how human robustness, $h_a$ for human accuracy and $h_p$ for human prediction similarity, is affected by increasing $\Delta_v$. For example, the orange line in Fig.~\ref{fig:metric-human-performance-integral} shows how human recognition accuracy changes as $\Delta_v$ increases when a transformation is applied. The procedure for obtaining $h_a$ and $h_p$ are as follows. First, $\Delta_v$ is computed for each image pair $\{(x_i,x_{i,j}’)\}$, and the pairs are sorted by $\Delta_v$ values into $r$ intervals, defined by $r+1$ equidistanced thresholds $t_k$, with $t_0=0$ and $t_r=1$. For our experiment, we selected $r=100$\red{TODO: update with new experiment}. For each interval, human accuracy and prediction similarity are calculated. Then, we reduce randomness and remove outliers by applying smoothing splines~\cite{koenker-94}. The final splines obtained with human accuracy is $h_a$, with human prediction similarity is $h_p$.

%These functions obtained from human robustness data can be reusable for different samples from the same distribution, or, intuitively, for images sharing the same characteristics, e.g., the same image resolution, the same objects, etc.~\cite{hu-et-al-22}. 


%For example, it is reusable across different sets of images of road scenes taken within the same geographic area using cameras with same the resolution and image quality.
%\begin{itemize}
%    \item Visual Change (IQA definition and how it's used to get human performance)
%    \item What is Human Experiment?
%\end{itemize}



==> sections/introduction.tex <==
\section{Introduction}
%\red{(Context)}
Neural Network (NN) models have been deployed in safety-critical systems, such as autonomous vehicles, which are subject to corruptions in their deployment environment~\citep{hu-et-al-22-b}, including 
varying brightness and weather conditions. 
Achieving robustness against such corruptions, \blue{i.e., corruption robustness,} is essential for the application of NN models in such safety-critical domains~\citep{hendrycks2019robustness}. NN models deployed in these domains automate tasks that are normally performed by humans, %and humans can generalize robustly across a wide variety of changes with minimum effort~\citep{Geirhos2018GeneralisationIH}. making
\blue{comparison of model robustness with humans a must for the applicability of models in such domains. } \purple{And we defined two novel metrics that can quantitatively compare model with humans. (?Bring up the subject earlier)}

%comparing model and human robustness is crucial for the applicability of models in such domains. 

%\red{NOTE: goal here is to show that we have this new idea of checking robustness and we conducted experiments to show this is promising, and in the meantime we provide tools to benchmark with our results. This can promote multiple directions of future research.}

%\red{
%\textbf{Human VS DNN robustness.} Merge the two paragraphs below to say a few points: 1) we are interested in corruption robustness through the lenses of comparison with humans (which is the average case), but so far this has been done with selected parameter values, and we wish to cover the full range; 2) as pointed out by our prior paper, DNNs might have better accuracy, but humans are better at preservation which we aim to check here; 3) retraining to gain insights.}

\noindent
\textbf{Human versus NN robustness.} 
%\subsubsection{Human VS NN robustness.}
%\red{what is corruption robustness, our key difference is human opinion, because humans sees wide and continuous, we have new way of testing robustness which is different from existing benchmarks.}
\blue{Corruption robustness measures the average-case performance of an NN or humans on a set of image corruption functions~\citep{hendrycks2019robustness}. Existing studies, including
out-of-distribution anomalies~\citep{Hendrycks2016}, benchmarking~\citep{hendrycks2019robustness,Hendrycks2019Natural}, and comparison with humans~\citep{hu-et-al-22,GeirhosNMTBWB21}, generally evaluate robustness against a pre-selected, fixed set of parameter values that represent varying degrees of image corruption.
However, parameter values cannot accurately represent the degree to which human perception is affected by image corruptions. For instance, using the same parameter to brighten an already bright image will make the objects harder to see; but will have the opposite effect on a dark image~\citep{hu-et-al-22}. In this paper, we revisit corruption robustness and introduce a new concept, \emph{visual-corruption robustness} (\robustness), that focuses on robustness relative to the impact of image corruptions on human perception instead of the parameter domain. 
Furthermore, humans can perceive and generalize across a wide and continuous spectrum of visual corruptions~\citep{Geirhos2018GeneralisationIH,VIF} ranging from the original image to the full distortion of all visual information. Therefore, test sets generated only with pre-selected parameter values can have insufficient coverage of the full range of visual corruptions, thus leading to potential biases in evaluation results. To address this gap, we also propose a method for test sets generation for testing the VCR and a robustness comparison with humans.} \purple{map this to the new points in the story}

%\blue{There are many studies in NN robustness against corruptions, robustness against out-of-distribution anomalies~\citep{Hendrycks2016}, corruption and perturbation robustness~\citep{hendrycks2019robustness,Hendrycks2019Natural}, and robustness comparison with humans~\citep{hu-et-al-22,GeirhosNMTBWB21}. These studies generally evaluate robustness against a pre-selected, fixed set of parameter values that represent varying degrees of image corruption. However, these pre-selected parameter values, being discrete, may not accurately portray the continuous range of visual corruptions perceptible to humans. Furthermore, these parameters do not necessarily reflect the degree to which a given corruption impacts human perception, leading to potential biases in evaluation results due to insufficient coverage of degrees of visual impacts in the validation set. To address these gaps, this paper revisits corruption robustness and introduces a new concept \emph{visual-corruption robustness} (\robustness), which leverages Image Quality Assessment (IQA) metrics to determine the degree of visual impact of image corruptions on human perception, focusing on average-case performance across a wide and continuous spectrum of visual corruption, then we test robustness with corrupted images ranging from the original image to the full distortion of all visual information perceived by humans.} 

\noindent
\textbf{Contributions and Outlook.} 
%\subsubsection{Contributions and Outlook.}
\blue{This paper proposes a novel definition of robustness, VCR, together with two novel human-aware NN evaluation metrics for assessing NN robustness in relation to humans. To do this, we conducted extensive experiments with 7,718 human participants on the Mechanical Turk platform on 14 commonly used image transformations. To foster future research, we open-sourced all human data as a comprehensive benchmark along with a Python toolbox that enables test set generation, testing, and retraining. Our experiments yield insightful findings about human and state-of-the-art (SoTA) NN robustness concerning accuracy, degrees of visual corruption, and consistency of classification, which can contribute towards NNs that better represent human perception. Additionally, we discovered classes of corruption transformations that affect human robustness similarly, (e.g., Shot Noise and Gaussian Noise in Fig.~\ref{fig:example}), while NNs react differently. Recognizing these classes can contribute to reducing the cost of measuring human robustness and elucidating the differences between humans and computational models.}

%The rest of the paper is organized as follows: Sec.~\ref{sec:related} reviews related work. Sec.~\ref{section:benchmark-generation} covers VCR and benchmark generation (Step~\RN{1} of Fig.~\ref{fig:intro-paper-design-flowchart}). Sec.~\ref{sec:experiments} describes how to identify similar transformations and obtain human performance data (Step~\RN{2} of Fig.~\ref{fig:intro-paper-design-flowchart}). Sec.~\ref{sec:eval-metrics} defines our two human-aware evaluation metrics (used in Step~\RN{3} of Fig.~\ref{fig:intro-paper-design-flowchart}). Finally, Sec.~\ref{sec:evaluation} evaluates our approach and Sec.~\ref{sec:conclusion} concludes. \red{TODO: update}
%\blue{
% This paper proposes 1) two novel human-aware metrics for measuring robustness as compared to humans \red{maybe a novel definition of robustness along with two metrics? for a wider and continuous range? parameter range difference? metrics that are closer to humans?}; 2) To assess VCR of NN compared with humans, we conducted extensive experiments with 7,718 human participants on the Mechanical Turk platform a human performance dataset for 14 commonly used image transformations involving a total of 7,718 Mechanical Turk participants; 3) a Python toolbox that enables benchmark generation, testing, and retraining}
%\red{ Outlook:  similar transformations as a discovery rather than a solution; outlook for improvements in DNN wrt to our definition; lessons learned. }


%\red{(Big problem + Robustness definition)} 
%There are many studies in assessing and improving model robustness focusing on adversarial robustness~\citep{Szegedy2014IntriguingPO}, robustness against out-of-distribution anomalies~\citep{Hendrycks2016}, model or data poisoning~\citep{Hendrycks2018}, robustness against image corruption or perturbations~\citep{hendrycks2019robustness}, robustness against altered images that are natural looking~\citep{Hendrycks2019Natural}, and robustness against visual change in images that do not affect human accuracy and predictions~\citep{hu-et-al-22}.
%In this paper, we extend the concepts of corruption/perturbation robustness~\citep{hendrycks2019robustness} and human-robust changes~\citep{hu-et-al-22}, and define a more generic form of robustness which we call \emph{visual-change robustness} (\robustness). Realistic environments
%in which autonomous vehicles need to operate contain  wide and continuous ranges of visual changes that can reflect both small perturbations (such as blurring in Fig.~\ref{fig:a}) and big image corruptions (such as in Fig.~\ref{fig:b}, where the corruption is visible and can affect human perception). 
%The \robustness{} is concerned with \emph{the average-case performance} considering \emph{all possible levels of visual changes} (i.e., from original image to the full distortion of visual information). \red{validity of test?}

%Before deployment, model robustness should be checked against transformations simulating the scene changes in the input~\citep{hu-et-al-22-b}, and existing benchmarks are developed for this purpose~\citep{croce2020robustbench, hendrycks2019robustness}. However, existing benchmarks generate tests using a few pre-selected transformation levels~\citep{hendrycks2019robustness}, which cannot cover the wide and continuous range of visual change that can be encountered during deployment and could result in bias in training and evaluation~\citep{hu-et-al-22}. Additionally, although robustness comparison with humans have been attempted~\citep{Geirhos2018GeneralisationIH}, existing benchmarks do not allow measuring how model robustness compares to humans. One reason is that %This is mostly because 
%human robustness is currently assessed through experiments with human participants for each image transformation~\citep{Geirhos2018GeneralisationIH}, which is an expensive process. 
%Therefore, this paper addresses this gap and develops a method, called \method, for benchmarking DNN \robustness{} against humans 1) across the full range of visual change and 2) at a cost reduced through experiment data reuse.
%\red{TODO: what's new}
 %a more refined and generic method for benchmarking DNN model \robustness{}.
%{\bf MC:  this thought should be earlier. \purple{[moved]}}


%\red{NOTE: paragraph and figure describing the process of the tool moved to supplementary}



%\red{(Summary of Contribution)}
%This paper contributes 1) two novel human-aware metrics for measuring model robustness as compared to humans; 2) a new benchmark for model robustness evaluation based on our proposed metrics; 3) a human performance dataset for 14 commonly used image transformations involving a total of 7,718 Mechanical Turk participants; 4) a method for transferring human performance data from one transformation to a class of transformations with a similar visual effect; 5) a Python library as well as a command line tool to automate image dataset benchmark generation, training, evaluation, and reuse of human performance data. 
%
%\red{(Experiment Results)} 
%{\bf MC:  do we need this paragraph?  can it be removed?}
%Using our approach, we compared robustness of state-of-the-art models (such as NoisyMix~\citep{NoisyMix} and AugMix~\citep{Hendrycks_AugMix}) on the corruption robustness dataset Imagenet-C~\citep{hendrycks2019robustness} leaderboard~\citep{croce2020robustbench} with humans. First, we identified two groups of similar transformation from the transformation library Albumentation~\citep{albumentation} and transformations used in existing approaches~\citep{hendrycks2019robustness, Geirhos2018GeneralisationIH}: 1) \purple{4 noise transformations}, \purple{e.g., Gaussian Noise} % Shot Noise, Impulse Noise, Gaussian Noise, Uniform Noise; 
%; 2) \purple{5 blur transformations, e.g., Gaussian Blur; and 3) 5 other non-similar transformations that change colour and brightness.} 
%Blur, Median Blur, Zoom Blur, Glass blur, Gaussian Blur, Defocus Blur, Motion Blur
%Through experiments, we showed that human robustness data is transferable between these similar transformations. %Then, with the above transformations and three other dissimilar transformations: Brightness, Frost and Color Jitter, 
%Along with two other non-similar transformations: Brightness and Frost
%. We showed that transformations in the two classes indeed resulted in similar human performance, thus human performance is transferable. 
%Then
%we show that %compared to the standard benchmark Imagenet-C, our method can generate a wider and more continuous distribution of visual changes in images; and 
%\purple{Then, by evaluating \robustness{} of state-of-the-art image classification DNNs, we showed that our method }
%\purple{Then, by }evaluating models with our method\purple{, we show that} can
%reveals insufficient robustness compared to humans for different levels of visual change in images, which is previously unseen in Imagenet-C.  We also report on experiments to show that low visual-change robustness can be mitigated through retraining with images we generated. 
%
%While we focused on image classification in this paper, our method can potentially be applied to other \purple{types of DNNs, such as object detection}. Data and implementation can be found at \red{\gitlink}.

%The rest of the paper is organized as follows: Sec.~\ref{sec:related} reviews related work. Sec.~\ref{section:benchmark-generation} covers VCR and benchmark generation (Step~\RN{1} of Fig.~\ref{fig:intro-paper-design-flowchart}). Sec.~\ref{sec:experiments} describes how to identify similar transformations and obtain human performance data (Step~\RN{2} of Fig.~\ref{fig:intro-paper-design-flowchart}). Sec.~\ref{sec:eval-metrics} defines our two human-aware evaluation metrics (used in Step~\RN{3} of Fig.~\ref{fig:intro-paper-design-flowchart}). Finally, Sec.~\ref{sec:evaluation} evaluates our approach and Sec.~\ref{sec:conclusion} concludes. \red{TODO: update}


\begin{figure}[t]
\centering
\scalebox{0.7}{
    \begin{tabular}{c c | c  c}
        %\toprule
         %& & & & \\
         \multicolumn{2}{c|}{\small Similar} &\multicolumn{2}{c}{\small Dissimilar}\\
          \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/7_shot_noise.JPEG}
         \caption{Shot Noise}
         \label{fig:a}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/66_gaussian_noise.JPEG}
         \caption{Gaussian Noise}
         \label{fig:c}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/77_motion_blur_c.JPEG}
         \caption{Motion Blur}
         \label{fig:d}
     \end{subfigure}
     &
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/transferability/33_brightness.JPEG}
         \caption{Brightness}
         \label{fig:e}
     \end{subfigure}
    \end{tabular}
}
%\vspace{-0.1in}
\caption{ImageNet images transformed with perceptually similar and dissimilar transformations.}
%The images are from Imagenet~\citep{ILSVRC2012} and the transformation is from Imagenet-c~\citep{hendrycks2019robustness}. }\
\label{fig:example}
%\vspace{-0.2in}
\end{figure}



%\begin{itemize}
%    \item (big context) First paragraph of imagenet-c: humans are good at certain type of robustness... although ML has been successful, they are still not robust (Geralisation: "Humans generalise across a wide variety of changes in the input distribution, such as across different illumination conditions and weather types.") -> realistic scene changes that can happen in the deployment environment (simulated by image transformations)
%    \item (big problem: ML robustnesss) Second paragraph of imagenet-c: existing work on robustness did ... + ..., in contrast, we focus on corruption robustness that studies... 
%    \item (smaller problem: corruption robustness) Existing work on corruption robustness (imagenet-c, robustbench, Generalisation...) ..., how we are different because we compare with humans. Additionally, our ICSE .... Therefore in this paper we propose a method that ..... (summary of the method) as shown in figure process
%    \item (intro of our method) first step ... , second step....
%    \item (summary of contribution) double check this. 
%    \item (experiment results) Through our experiments, (see Natural adversarial example) we demonstrate ??? of our method through experiments with ??? models, comparison with ??? benchmarks, we show that our tool is ???? better, ??? effective at ??? etc. 
%    \item (paper organization) The rest of the paper is structured as follows: ...
%\end{itemize}


%Computer Vision (CV) models have been shown to be not robust against small changes in input images~\citep{Szegedy2014IntriguingPO}. While human visual system is inherently robust, as it has developed over time to tolerate a wide range of variations in the visual input. 
%Achieving human-level vision robustness is an important goal for computer vision and machine learning methods, as they are widely deployed in so many areas, including safety-critical fields like autonomous driving. ML models should to be at least as reliable as human to safely replace human in these safety-critical fields~\citep{hu-et-al-22}.

%\purple{add robustness against humans in existing work. We define more generic robustness first (range of changes that are visual to humans); until threshold ... also useful beyond that ...  }

%\purple{To check such robustness, existing work is not enough. What most benchmarks don't do is also to compare with human because the cost is high. In this paper, addressing these challenges, we propsoe a generic method for creating validation datasets to benchmark \robustness. }

%\purple{Introducing our method: we propose a way to generate images, we also propose methods to compare with humans and a way to reduce that cost.}


%for considering natural visual changes that can be encountered in the deployment environment, such as brightness and snow, we call it \emph{\robustness}. In reality, the environment contains a wide range of visual changes that can be both small perturbations and big image corruptions. For example, as shown in Fig.~\ref{fig:example}, in Fig.~\ref{fig:b} the amount of frost is a small perturbation, a visible corruption as in Fig.~\ref{fig:c} and even more corruption in Fig.~\ref{fig:d}. All these levels of frost can be encountered by an autonomous driving vehicle, thus \robustness{} focuses the average-case performance of a model facing different levels of visual changes.
%\purple{OR put human (us) here to compare. Additionally, a new way is... since CV replaces human, also define robustness with humans, both accuracy and predictions ... take a step further and We propose a new generic robustness definition for this (we shouldn't stop at those that don't affect humans ... ). The range of changes we cover which is used in definition of robustness. }

%\red{TODO: very similar to corruption robustness https://arxiv.org/pdf/1903.12261.pdf} 
%In contrast, our assessment of the ML models involves measuring their robustness \emph{compared to human performance}.
% Specifically, we introduce \red{BenchmarkName} benchmark that measures the performance difference between ML models and humans. 
%The accuracy and predictions of the models should not be affected by both {\bf MC : both or either?} small perturbations and big image corruptions that do not affect human performance. As shown in Fig.~\ref{fig:example}, level of frost that can be encountered by an autonomous driving vehicle can be  minimal as in Fig.~\ref{fig:b}, or a visible corruption as in Fig.~\ref{fig:c} and even more corruption in Fig.~\ref{fig:d}.  {\bf MC:  why do we start with Figure 3?} We call this \emph{\robustness} .  {\bf MC:  what specifically do we call robustness?}
%Most work on robustness in CV methods focus on measuring the accuracy of image classification models when changes are present. This is the traditional way of measuring model's performance, but doesn't reflect the distance of performance comparing to humans.
%In contrast, we focus on evaluating models' robustness comparing to humans. 

%\red{(Smaller Problem)}

%\purple{Here we talk about checking such robustness: coverage problem and experiment expense}
%\purple{(problem with existing approach) To check we need benchmark} 

%\purple{To assess robustness, we define a method for benchmarking. problem with existing benchmark, we aim to have coverage. In order to have coverage we need a range, we define this range using humans, visual is defined with human performance. problems with existing methods with humans.  }

%\purple{CV robustness should be compared with humans. problem with existing benchmarks, }

%In reality, humans are exposed to many different levels (continuous instead of discrete) of visual change. Thus, to compare with human performance, we have to cover a wide, continuous range of visual changes rather than using a few pre-selected transformation levels which could result in bias in training and evaluation. Current methods are not capable of testing models against the visual changes humans are exposed to. Our evaluation method covers the entire range of visual changes by uniformly sampling from the entire domain of transformation parameters. Both human and ML models are evaluated on the samples, providing more realistic testing scenarios.  


%Since CV models are deployed in safety-critical systems that automate tasks that are normally performed by humans, and humans can generalize robustly across a wide variety of changes with minimum effort~\citep{Geirhos2018GeneralisationIH}, another view for model robustness is that models should \emph{at least be robust to changes that do not affect human performance~\citep{hu-et-al-22, Firestone26562}}. However, the degree of changes included in existing benchmarks for checking robustness~\citep{hendrycks2019robustness, croce2020robustbench} is either too small (only included either images with human-imperceivable adversarial changes~\citep{croce2020robustbench}) or does not cover the domain of visual changes (images transformed with five pre-selected parameter values for each image transformation~\citep{hendrycks2019robustness,Geirhos2018GeneralisationIH})~\citep{hu-et-al-22}, which could cause bias in the resulting models that are evaluated on these pre-selected parameters. Therefore, in this paper, we address this gap of benchmarking model robustness against real-world scene changes compared to human robustness. 

% \blue{TODO: add When comparing with humans, we need a different type of coverage. 
% We need to be explicit about this and say what we do. 
% Current methods don’t have a way to do that kind of coverage. 
% Why is coverage is needed? How we do it. } 

% \blue{TODO: add the issue of reduce the need for costly experiment if transfer is possible here}
%Human robustness is currently assessed through experiments with human participants per image transformation~\citep{Geirhos2018GeneralisationIH}. Hu et. al~\citep{hu-et-al-22} proposed a method that given an image transformation, measures the threshold of level of visual changes in the images that does not affect human performance in image classification. This is achieved with two concepts -- correctness-preservation and prediction-preservation, where correctness-preservation requires correct predictions after transformation and prediction-preservation requires the same prediction after an image is transformed. 
% \blue{TODO: correctness-preservation and prediction-preservation (accuracy and human predictions)}.
%However, beyond such threshold, as more changes are introduced, human performance gradually decreases  rather than dropping drastically.
%Therefore, leveraging human performance for different level of changes, in this paper we propose a method for benchmarking model robustness compared to human performance by generating benchmark datasets that covers different levels of visual change in the images. While there are many types of image transformations and human experiments are expensive, it would be efficient if we can reuse existing experiment results for a new transformation when two are similar. In this paper, we also propose a method to determine whether two transformations are similar and whether the human experiment results are reusable.
%As shown in Fig.~\ref{fig:intro-paper-design-flowchart}, given a transformation and an image dataset, it first generates a benchmark dataset with transformed images (step 1) to evaluate model robustness against humans. Then using the benchmarking dataset, we evaluate model robustness (step 5) with two new metrics: $M_a$ that measures how close model performance is to humans, and $M_b$ that measures how much a model can exceed human performance. \red{TODO: need way better names + prediction-preservation ones}.  

%Additionally, since the human performance used as reference has to be obtained through experiments with human participants per transformation, we also provide such data for a few commonly used transformations: \red{TODO: select transformations} (step 2). Also, obtaining human performance data for every single image transformation (step 3) is not only expensive but time-consuming as well. However, some transformations have very similar visual effects and they affect human recognition performance similarly. For example, as shown in Fig \ref{fig:compare-blurs}, images transformed with Gaussian Blur and Median Blur have very similar visual effects on humans. Therefore, human performance data for Gaussian Blur can be transferred to Median Blur. We propose a method that generalizes existing human performance data obtained for one transformation to a class of transformations with similar visual effects. 
%For such transformations, human data can be reused (step 4).  Thus, following this, to save time and resources we also propose a method to decide whether two transformations are visually similar enough such that human data can be reused. 
%\purple{update with experiment plan: how transformations are selected, how models are selected and how retraining happened. What our results showed. }
%\textbf{TODO Placeholder: Experiment Results Section.} %Experiment results show that ...
%Through evaluation with existing robustness benchmark Imagenet-c with models on the robustbench model zoo, we showed that \red{TODO: temp} our method generates a fairer distribution of visual changes in images, and can effectively compare and improve model robustness compared to humans.
%\blue{Some relevant sentences from~\citep{Geirhos2018GeneralisationIH} that we can use: First, we assess how top-performing DNNs that are trained on ImageNet, GoogLeNet [38], VGG19 [39] and ResNet-152 [40], compare against human observers when tested on twelve different distortions such as additive noise or phase noise (see Figure 2 for an overview)—in other words, how well do they generalise towards previously unseen distortions.2 In a second set of experiments, we train networks directly on distorted images to see how well they can in general cope with noisy input, and how much training on distortions as a form of data augmentation helps in dealing with other distortions.}%\red{Question: if results are discussed along with the contribution above, what do you want to say here? A summary of results?}



%\noindent==================================\\
%V1 Below\\
%==================================

% \begin{itemize}
%     \item Talk about robustness of human and ML models.
%     \item Summary of each of the following topic.
% \end{itemize}


%Machine learning evolved so quickly in recent years that its applications became an inseparable part of our daily life. Neural Networks, as the state-of-the-art technique in this field gained lots of attentions and were applied to all kinds of areas, including safety critical fields like autonomous driving, where the reliability and robustness of ML models is crucial. In this paper, we are going to focus on image classification, the most fundamental computer vision task.

%Computer Vision (CV) is widely deployed in safety-critical systems in different areas, such as autonomous vehicles. CV models in such systems represent the critical function for the overall system safety, which raised safety concerns as undesired behaviors can lead to fatal accidents~\citep{zhang2018deeproad}. 
%However, CV models have been shown to be not robust against changes in the input images~\citep{Szegedy2014IntriguingPO}. This fact has lead to abundant studies in assessing and improving model robustness~\citep{hendrycks2019robustness}, most specifically focusing on measuring the accuracy of image classification models when changes are present. 

%Since such models are deployed in systems that automate tasks that are normally performed by humans, and humans can generalize robustly across a wide variety of changes with minimum effort~\citep{Geirhos2018GeneralisationIH}, another view for model robustness is that models should be robust to changes that do not affect human performance~\citep{hu-et-al-22}. Hu et. al~\citep{hu-et-al-22} proposed a method that given an image transformation, measures the threshold of level of visual changes in the images that does not affect human performance in image classification through experiments with human participants. However, beyond such threshold, as more changes are introduced, human performance rather than dropping drastically, gradually decreases. Therefore in this paper, leveraging human performance for different level of changes, we propose a method for benchmarking model robustness compared to human performance by generating benchmark datasets with different levels of visual change in the images. 

%We propose a method \red{TODO:name of the method}, as shown in Fig.~\ref{fig:intro-paper-design-flowchart}, that given a transformation, a image dataset, first generates a benchmark dataset with transformed images (step 1) to evaluate model robustness against humans. Then using the benchmarking dataset, we evaluate model robustness (step 5) with two new metrics $M_a$ that measures how close model performance is to humans and $M_b$ that measures how much a model can exceed human performance. \red{TODO: need way better names} Additionally, since the human performance used as reference has to be obtained through experiments with human participants per transformation, we also provide such data for a few commonly used transformations: \red{TODO: names} (step 2). Also, obtaining human performance data for every single image transformation (step 3) is not only expensive but time-consuming as well, we also leverage the fact that certain transformations have very similar visual effects that they affect human recognition performance similarly. For such transformations, human data can be reused (step 4). For example, as shown in Fig \ref{fig:compare-blurs}, different types of blurring can have small perceptual difference and similar impact on humans. Thus, following this, to save time and resources we also propose a method to decide whether two transformations are visually similar enough such that human data can be reused. 


%In order for ML to replace humans confidently in safety-critical fields such as autonomous driving, ML models are expected to be at least as reliable/robust as human\citep{DBLP:journals/corr/abs-2202-03930}; while current ML models are still not as robust as humans (TODO: add some evidence?). Neural Networks learn from experience, i.e. remembers features they have seen (TODO: add some citations here). NNs lack the ability to generalize to unseen input (TODO: add some citations here). Current techniques for improving robustness includes image augmentation/corruption (ImageNet-C, Cifar10-C) \citep{hendrycks2019robustness} \citep{DBLP:journals/corr/abs-1807-01697}, adversarial training, etc. which essentially try to feed more types of inputs to a model to make NNs learn more features, thus more robust. The evaluations of ML models are usually based on accuracy-based metrics (RobustBench: Adversarial robustness benchmark\citep{DBLP:journals/corr/abs-2010-09670}), (TODO: add more related work of metrics, or add in related work section) which doesn't really reflect ML models robustness with respect to human performance. Accuracy is like an absolute measurement of performance, but we also need a relative measurement to compare the distance between ML performance and human performance. 

%Our idea for measuring robustness relative to human is to introduce a new metric that involves human performance. In this paper, we propose a new metric and a benchmark generating method for evaluating ML models performance relative to humans given an image dataset and a transformation type. The metric is based on human tolerated range on image transformations, i.e. the range of perturbation humans can tolerate without making mistakes. It measures and compares how robust ML models are comparing to humans.
%As the workflow shown in Figure \ref{fig:intro-paper-design-flowchart}, given an image dataset and a transformation type, we first retrieve human performance from new experiments or existing data; then evaluate an ML model with our generated benchmark dataset and proposed metric that is capable of measuring the distance between ML performance and huamn performance. Eventually we can evaluate how robust a ML model is comparing to humans.


% Our idea for measuring robustness relative to human is to introduce a new metric that involves human performance. The metric is also based on accuracy, but takes human performance into account. IQA (Image Quality Assessment) is a method for measuring visual quality change between 2 images (TODO: make sure this is correct). Given a transformation type, by applying different levels transformations on images, we get a range of IQA values. Then by measuring humans' performance (accuracy) on different levels of IQA values, we can plot a performance curve whose x-axis is IQA value and y-axis is human accuracy. See Figure (TODO). We can calculate the area under the curve by taking integral on it. The area under the curve represents the performance, the larger the better. Similarly we can generate a performance curve for an ML model. By comparing the 2 curves we can visualize the performance distance between ML model and human. The difference between the 2 areas numerically measures the performance difference; and by subtracting the area difference by human performance area, we get the relative performance difference between human and the given ML model.

%Human performance data must come from real human experiments, which is not only expensive but also time consuming. We can't expect humans to classify images as fast or as much as ML models can do, and there are infinitely many transformation types. For each transformation type and each type of task, we may have to conduct an experiment for measuring human performance. However, for similar transformation types which have similar effects on human performance, we can potentially reuse existing human performance data. Thus, we also propose a method of reusing human performance data from one transformation type to another similar type. With the assumption that, "if humans cannot tell the difference between two transformations, the two transformations will affect human recognition performance similarly", we can reuse human performance data from one transformation type on another if they are similar enough. We define "similarity" as, "whether humans can tell the perceptual difference between two transformations".


%Our main contributions can be summarized as follows
%\begin{itemize}
%    \item We propose a novel metric for measuring model robustness comparing to humans' performance. TODO: talks about what's achieved with evidence from experiment results. 
%    \item We provide sample human performance data for (Placeholder: transformation types we will conduct experiment on).
%    \item We propose a method for reusing human performance data, that transfers existing human performance data of one transformation type to another, saving resources from conducting excessive experiments. With thorough experiments, we showed that similar transformation types result in similar human performance, and human performance is transferable.
%    \item We provide a Python library as well as a command line tool to automate image dataset benchmark generation, training, evaluation, and reusing human performance data. Making evaluation easier for researchers.
%\end{itemize}
    

%\textbf{TODO Placeholder: Experiment Results Section.} %Experiment results show that ...
%Through evaluation with existing robustness benchmark Imagenet-c with models on the robustbench model zoo, we showed that ... \red{Question: if results are discussed along with the contribution above, what do you want to say here? A summary of results?}
%We focused on image classification in this paper, while this technique could potentially be applied in more areas.

%The rest of the paper is organized as follows ... \red{TODO: also fill this in with the plan we currently have of different sections}





==> sections/overview.tex <==
\section{Overview}

\begin{itemize}
    \item Assumptions
    \item Motivating Example (e.g. sample)
    \item Flow chart (includes all sections below, transfer $\rightarrow$ image gen $\rightarrow$ metric (eval) $\rightarrow$ retrain)\\
        \indent\quad Retraining with reliability-cli generated data and proposed metric as criterion
    \item Retraining\\
        \indent\quad How to retrain in general
    \item Tool support (link to GitHub)
    
\end{itemize}

==> sections/rebuttal.tex <==

\section{\blue{Temporary Rebuttal Section}}
\subsection{Model Table}




\subsection{Q: Why 200ms for human:}
A: According to Generalisation in humans and deep neural networks \cite{Geirhos2018GeneralisationIH}, "standard DNNs only use feedforward computations at inference time, while recurrent connections are ubiquitous in the human brain. In order to prevent this discrepancy from playing a major confounding role in our experimental comparison, presentation time for human observers was limited to 200 ms."

\subsection{Please briefly discuss the qualification tests and sanity checks aimed to filter the participants.}
For qualification, we give the participant a small sample experiment with 20 images using the same set up as the actual experiment. These images are hand picked by us to be easy to classify (big, clear object in the center). The goal here is to make sure that the participants fully understand what they are supposed to do. 
Additionally, we hid sanity images, which are also easy images, inside each experiment and monitored the accuracy on those images. The participants are expected to correctly classify these images. The goal for sanity images is to filter out participants who selected random classes.  

\subsection{A curious question, What is the total number of participants before the filtration process?}
Unfortunately we do not have a number for this, we did not keep the results of those who did not pass sanity and qualification test. 

\subsection{Are same images seen by each human participant?}
We designed our experiments so that the same image (corrupted or not) is never shown to the same human participant.

\subsection{40 Bins question. In extreme case when bin number is 1, how to ensure the coverage is reasonable?}

A similar choice in the Pascal VOC challenge paper is, the precision-recall curve is plotted using 10 evenly divided intervals, rather than selecting a single bin. We chose 40 as a higher number to depict coverage on a finer scale. 

\subsection{ImageNet-CCC and ImageNet-3DCC}

ImageNet-3DCC is not a continuous dataset, they incorporate geometry info in the dataset, so we didn't compare.

ImageNet-CCC is indeed continuous. We didn't compare with it because: 1. it's very new. GitHub repo code was from 6 months ago. 2. No dataset available to download online, generation code on GitHub is not runnable.

==> sections/transferability.tex <==
\section{Transferring Human Robustness Data}
\label{sec:transferability}
In this section, we introduce our method for identifying \emph{similar} transformations for transferring data (Step~III of  Fig.~\ref{fig:intro-paper-design-flowchart}). This is implemented as part of \method{} to allow users to check whether new human data is needed to analyze a new transformation. 

%\noindent
%\textbf{Identify Classes of Similar Transformations.}
%\begin{itemize}
%    \item How do we define similarity
%Different image transformations can impact human perception differently, e.g., changing colour, brightness, thus human robustness is typically measured per transformation~\cite{hu-et-al-22}. Conducting experiments to obtain human robustness data for every new transformation is expensive and time-consuming. However, for transformations that impact human perceptions \emph{similarly}, human robustness data can be transferred between the transformations.

Different transformations change different aspects of the images, e.g., image colour, contrast and the amount of additive visual noise, and thus affect human perception differently~\cite{Geirhos2018GeneralisationIH}. Also, multiple different transformations can be implemented for the same visual effect, such as Gaussian blur and Glass blur for image blurring as shown in Fig.~\ref{fig:example}. Although the difference between Gaussian blur and Median blur can be picked up by complex DNN models, an average human %without high computational power 
would struggle to distinguish between the two. Therefore, for a specific visual effect, we say that there exists a class of transformations implementing it if an average human is unable to tell them apart. We call  transformations in the same class \emph{similar}. We postulate that since similar transformations, by definition, affect human perception similarly, they would affect human robustness similarly as well, and thus 
%Similar transformations affect human perception similarly, therefore should affect human robustness similarly. As a result, 
human data for one transformation can be transferred to other similar transformations in the same class. 

%    \item How to check similarity with humans?
%    \item Distribution of image sampling
To identify whether two transformations $T^1_X$ and $T_X^2$ are similar, we need to determine whether the difference between them is distinguishable to a human. This can be done through a small set of experiments. Participants of such experiments are expected to have basic knowledge of image transformations. 
%
%To identify whether two transformations are similar, two things need to be checked: whether humans are able to tell the difference between two transformations, whether the degree of changes is distributed similarly. 
%This can be identified with a small set of experiments with a human. 
First, %for each transformation $T_X\in \mathbb{T}$ with the parameter domains $C$ and distribution $P_C$, 
%$N$ original images $x_i \sim P_X$ are randomly selected and 
$N$ transformed images $x'$ are generated by transforming $x\sim P_X$ with $c \in C$, that is $x' = T_X(x, c)$. For efficiency, all changes in $x'$ should be clearly visible to the participants, thus \purple{in this paper} we use that $\Delta_v(x, x') >= 0.8$ {\bf MC:  why this number? \purple{addressed}} for all $x'$, \purple{this number can be adjusted as needed}. %Then, we check the similarity of every $T_X^1, T_X^2 \in \mathbb{T} \times \mathbb{T}$ in the process of the experiment. 
The participants are shown two images side by side: $x'^1$ transformed with $T_X^1$ and $x'^2$ transformed with $T_X^2$.  They  are asked whether the pair of images presented are transformed with the same transformation, i.e, whether they think $T_X^1 = T_X^2$. The experiment includes the same number of image pairs where $T_X^1 = T_X^2$ and $T_X^1 \neq T_X^2$. If $T_X^1$ and $T_X^2$ are similar, the participant would only be able to distinguish them with close to random accuracy, which is $0.5$. {\bf MC:  why this number? \purple{because the experiment is distinguishing two transformations at a time}} For each pair of $T_X^1$ and $T_X^2$, we use a binomial test with $p=0.5$ to test whether the Null hypothesis `human cannot correctly distinguish $T_X^1$ and $T_X^2$, i.e., accuracy$=0.5$' holds for the human opinion we observed in the experiments. The Null hypothesis is accepted if p-value is $\geq 0.95$, meaning that the participant cannot tell the two transformations apart, and thus they are similar. This is an indication that human robustness data can be reused for these two similar transformations. 
A transformation belongs to a class of similar transformations if it is similar to every transformation in the class. 

%The two $x_{i,j}'$ can be transformed with the same or different transformation and equal amount of such pairs are included in the experiment. 
% Then, the generated images $x_{i,j}'$ are randomly paired up and the participants are shown two $x_{i,j}'$ 
%Then images generated are randomly paired up and shown to the humans as pairs. For each pair of transformations, equal amount $M$ of same transformed pair and differently transformed pair are included. Humans are asked whether they think the pair of images presented are transformed with the same transformation. 
%After collecting human opinion, a binomial test is used to check whether the human can tell the different transformations apart with better than random accuracy ($0.5$). \red{maybe rather than pairs, it should be a set to represent distribution?} 

%Since the entire experiment is fully randomized, there is no bias in the results with the authors. 
%To avoid bias, all transformations and images are fully randomized. 
%This part is implemented as an addition to our tool. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Archive %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%CV models due to its high complexity and computational power, can pick up more information in images than human perception.
%Different transformations can be affecting the same aspect, e.g., Gaussian blur and Median blur as shown in Fig.~\ref{fig:compare-blurs}, that can confuse CV models, but an average human cannot detect the difference between the two transformations.\red{TODO: a generalized class of transformations} 
%Therefore, we call such transformations \emph{similar} as they have the same visual impact on human perception. \red{TODO: does distribution matter?}
%    \item Assumption: if human can't tell the difference between 2 transformations, the effects of the transformations should be similar\\
%For such similar transformations, human perception is affected similarly, therefore how the changes affect human robustness should also be similar and thus human data can be transferred.

%Following procedures in Sec.~\ref{sec:experiments}, for each of the selected transformations, we sample 1000 transformed images $x_{i,j}’$ from the ILSRVR'12 dataset, and have each image labeled by five humans. To achieve this, we divide the 1,000 (transformed images) $\times$ 8 ($\#$considered) transformations into batches of 20 images.Each batch is shown five times to different participants using the platform Amazon Mechanical Turk.We include qualification tests and sanity checks aimed to filter out participants  misunderstanding the task and spammers~\cite{Papadopoulos-et-al-2017}, and only consider results from participants who pass both tests.\red{TODO: update with real experiment} As a result, for the ILSVRC'12 image classification task, we use $\{x_i\}$ with 13,000 car images and same number of non-car images, and collect human predictions for 40,000 ($= 5 \times 8 \times 1,000$) transformed images and the same number of the original images, for a total of 80,000 predictions. 
